Interpreting Instrumental Variable Estimands with Unobserved Treatment Heterogeneity: The Effects of College Education

Many treatment variables used in empirical applications nest multiple unobserved versions of a treatment. I show that instrumental variable (IV) estimands for the effect of a composite treatment are IV-specific weighted averages of effects of unobserved component treatments. Differences between IVs in unobserved component compliance produce differences in IV estimands even without treatment effect heterogeneity. I describe a monotonicity condition under which IV estimands are positively-weighted averages of unobserved component treatment effects. Next, I develop a method that allows instruments that violate this condition to contribute to estimation of treatment effects by allowing them to place nonconvex, outcome-invariant weights on unobserved component treatments across multiple outcomes. Finally, I apply the method to estimate returns to college, finding wage returns that range from 7\% to 30\% over the life cycle. My findings emphasize the importance of leveraging instrumental variables that do not shift individuals between versions of treatment, as well as the importance of policies that encourage students to attend "high-return college" in addition to those that encourage "high-return students" to attend college.

==> Lambda_hat.tex <==
\begin{small}\begin{tabular}{l  c  c|}
\hline
\textbf{Age} &\textbf{Component 1 Effect}&\textbf{Component 2 Effect}\\\hline
\textbf{25}&5.55&9.56\\\hline
\textbf{26}&4.91&8.54\\\hline
\textbf{27}&3.84&5.20\\\hline
\textbf{28}&-0.89&-0.79\\\hline
\textbf{29}&4.91&5.36\\\hline
\textbf{30}&5.92&5.56\\\hline
\textbf{31}&8.50&6.03\\\hline
\textbf{32}&7.52&6.20\\\hline
\textbf{33}&8.86&6.98\\\hline
\textbf{34}&8.70&5.79\\\hline
\textbf{35}&6.80&3.11\\\hline
\textbf{36}&5.07&1.02\\\hline
\textbf{37}&3.20&-1.47\\\hline
\textbf{38}&1.21&-3.90\\\hline
\textbf{39}&0.25&-6.08\\\hline
\textbf{40}&3.69&-4.40\\\hline
\textbf{41}&7.96&-2.12\\\hline
\textbf{42}&12.46&0.67\\\hline
\textbf{43}&15.47&2.22\\\hline
\textbf{44}&16.96&2.43\\\hline
\textbf{45}&19.40&3.93\\\hline
\textbf{46}&22.11&5.72\\\hline
\textbf{47}&24.59&7.18\\\hline
\textbf{48}&26.38&8.19\\\hline
\textbf{49}&28.02&9.16\\\hline
\textbf{50}&23.00&15.02\\\hline
\end{tabular}
\end{small}

==> Sections/Conclusion/Conclusion_v1.tex <==
\section{Conclusion}

Determining individual level heterogeneity in treatment effects is a major focus in both econometric theory and applied research. This paper draws attention to the similar importance of unobserved heterogeneity in treatments. At a high level, this paper contributes to discussions of both instrumental variables and reduced form results in empirical applications by offering a potential explanation for differences between studies and identification strategies - that different estimators identify effects of different unobserved component treatments. In addition to explaining differences between empirical results, unobserved treatment heterogeneity is also relevant for policy, as some component treatments may have substantially larger/smaller effects than others. 

Additionally, this paper describes a treatment-level net monotonicity condition on instrumental variables that is sufficient for the interpretation of standard IV estimates as positively-weighted averages of unobserved treatment effects. It also provides a method for researchers to use to estimate effects of unobserved treatments when there are multiple outcomes and valid instruments. This method is helpful for investigating heterogeneity in treatments for its own sake, as well as permitting instruments that are exogenous and independent, while violating monotonicity conditions, to contribute to estimation.

Finally, I would be remiss if I did not end with a discussion of similarities and differences between unobserved treatment effect heterogeneity, especially in the the context of the local average treatment effect framework, and unobserved treatment heterogeneity. Broadly, any trait of an individual that affects their returns may manifest through unobserved choices about their preferred version of the treatment, while any variation between individuals in unobserved treatment choices may be perfectly determined by unobserved preexisting characteristics. The differences in policy implications, however, are substantial. In the specific case of returns to college, the possibility that even a portion of the negative returns for a large minority of the population \citep{cunha2005separating} could be driven by unobserved treatment heterogeneity opens the door to potentially massive policy implications for targeted incentives on high-return types of college for these individuals. I leave the ambitious task of separate identification of treatment effect heterogeneity and treatment heterogeneity to future work.

==> Sections/Data/Data_v1.tex <==
\section{Data}
I estimate returns to college with the factor-augmented treatment effects model described above using data from the National Longitudinal Survey of Youth 1979 (NLSY79).
The NLSY79 follows a group of 12,686 individuals who were between the ages of 14 and 22 in 1979. Respondents were surveyed annually for the first 15 years and biennially afterwards. Survey responses include information on years of education, earnings, geography of residence, and a wealth of auxiliary information. In addition to meeting the requirements of my model of containing multiple instruments and outcomes, this dataset is attractive because it has been used extensively in the literature on returns to education, which helps us to emphasize my methodological contributions by holding fixed some other potential explanations for similarities and differences in results. In particular, I use the same sample of white males that was used by \cite{carneiro2011estimating}, matched with longitudinal wage data constructed according to the procedure described in \cite{ashworth2017changes}.

The composite treatment of interest is college attendance as of age 25. Estimating my model requires multiple outcomes and instruments, as shown in expression (\ref{Identification_condition}). The longitudinal nature of the NLSY allows us to set $j=t$ for $t=25,\dots,40$ and rely on wage outcomes over the lifecycle to identify the model.%
% \footnote{Panel data is not required for estimation if a sufficient number of outcomes are available in a single time period. Repeated cross-sections can also be used.}
% I expect 2SLS effects of education on wages to be correlated over time for each IV, which may threaten identification if they are collinear or nearly so. To address this concern, I also plan to include fertility, marriage, and health responses in each available time period as outcomes in a future version of the paper.%
\footnote{Researchers considering using this method in other applications should rarely be deterred by a lack of outcomes. Even if economically meaningful outcomes are sparse in a given dataset, it is possible to estimate the model using outcomes that lack obvious economic significance but nonetheless contribute to identification.}

 I  use several instruments that are established in the literature on returns to education. They are an indicator for the presence of a college in county of residence at age 14, average tuition of public colleges in the county of residence at age 17, and average wages in the county of residence at age 17.% , and the unemployment rate in the state of residence at age 17.%
\footnote{
The unemployment rate in the state of residence at age 17 is another commonly used instrument. I have opted to exclude it because it is extremely weak compared to the other instruments.
}
That each of these variables contributes to the college attendance decision is intuitive as well as testable. I discuss instruments separately in terms of excludability and intuition for the type of college they identify.

The presence of a college in the county of residence at age 14 has been used as an instrument for education by \cite{card1993using, kane1995labor, kling2001interpreting, currie2003mother, cameron2004estimation, carneiro2011estimating}; and \cite{mogstad2021identification}. I expect the presence of colleges in the county of residence to primarily influence education by encouraging students to attend college through a cost reduction mechanism. 
% Insofar as colleges near residences of survey respondents are representative of colleges in general, this instrument may identify the type of education associated with attending the average college. 
If cost reduction is more important for students inclined toward particular types of college education, such as majors \citep{altonji2012heterogeneity} or quality \citep{black2006estimating}, then this IV will identify the effects of such types of education. The validity of this instrument is threatened by correlation between college presence and students' ability, as noted by \cite{carneiro2002evidence} and \cite{cameron2004estimation}. To address this, I control for a measure of ability (the Armed Forces Qualification Test, AFQT), following \cite{carneiro2011estimating}.

Local tuition costs have been used as an instrument for education by \cite{kane1995labor}, \cite{cameron1998life}, \cite{cameron2001dynamics}, and \cite{carneiro2011estimating}. This is similar to local labor market conditions in that it may be correlated with unobserved ability, such as if expensive colleges produce different externalities for the local community than cheap colleges. I control for mother's years of education, permanent local labor market conditions, and AFQT to address this concern. I expect this instrument to affect educational attainment through similar channels as the presence of a college in the county of residence. By defining an unobserved component of education in terms of one of these instruments, I can empirically check if my model describes the other instrument as placing a high weight on this component, which is an intuitive check for the validity of my model.\footnote{A possible explanation for these instruments driving education through different channels is that tuition costs drive the type of education that pecuniary-cost-sensitive students are inclined toward, while the presence of a nearby college drives the type of education that nonpecuniary-cost-sensitive students (for instance, those with high psychic costs of distance from family) are inclined toward.}



Local wages have been used as explanatory variables for educational decisions by \cite{cameron1998life}, \cite{cameron2001dynamics}, \cite{cameron2004estimation}, and \cite{carneiro2011estimating}. Following \cite{carneiro2011estimating}, I use the average values of these at age 17 at the county and state level, respectively, as instruments for college attendance. Because local labor market conditions may contribute to outcomes through channels other than education, I include permanent values of these as controls in outcome equations as well as selection equations, while including these values at age 17 only in selection equations. It follows that I effectively am using temporal deviations from average in local labor market conditions at age 17 as instruments. Good labor market conditions could resolve credit constraints, driving price sensitive students to attend colleges, which may be relatively cheap or low quality, or they could induce students to drop out of high school or not attend college due to improving outside options. 

 I  use several variables as controls, which is common in the literature. They are number of siblings, 
permanent local unemployment, permanent local log wages, a binary indicator for urban residence at age 14, average wages in county of residence in 1991, average unemployment in county of residence in 1991, year of birth indicators, mother's years of education, and the Armed Forces Qualifying Test score. Statistics on the variables I use are shown in Table \ref{tab:descriptives}.
% I expect to include a richer set of controls in a future version of the paper.

\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Summary Statistics}
\label{tab:descriptives}
\begin{tabular}{l*{3}{c}}
\midrule
\input{Figures_Tables/descriptive}
% \hline
% \hline
\end{tabular}
\begin{minipage}{1\linewidth}
\smallskip
\footnotesize
\emph{Notes:} Means and standard deviations for white males in the National Longitudinal Survey of Youth 1979 sample. AFQT corrected for years of schooling at the timing of test-taking. Permanent log wages and unemployment are calculated as average values from 1973 to 2000 for the county of residence at age 17. 
\end{minipage}
\end{table}

==> Sections/FATE/FATE_v1.tex <==
\section{Factor Augmented Treatment Effects}

 I  apply the insights above to estimate returns to unobserved components of college education. It is likely that unobserved components of college may manifest in the intensive margin, such as if students alter the composition of classes they choose to take while in college, or if they modulate their study intensity across classes. To capture this, I model the unobserved component treatments as continuous for my application, despite the binary nature of the observed composite treatment.

For an individual indexed by $i$ among $N$ individuals and an outcome indexed by $j$ among $J$ outcomes, the model describes $L$ endogenous unobserved components of college education, $F_{i}$, affecting an outcome, $Y_{ij}$, as follows
\hfill
\begin{equation}\label{Second_stage_true}
% \begin{gathered}
Y_{ij} = X_{i}\beta_j+F_{i}\lambda_j+\epsilon_{ij}
% F_{ij} = Z_{i}\Gamma_{}+U_{i}
% F_{j} = X_{}\Psi_j+Z_{}\Gamma_{}+U_{j}
% w_{j} = F_{j}\Lambda_j+\epsilon_{j} \\
% F_j = Z_j\Gamma_{}+u_{j}
.
% \end{gathered}
\end{equation}
Outcome-specific marginal effects of $F_{i}$ ($1 \times L)$ on scalar $Y_{ij}$ are given by $\lambda_j$ ($L \times 1$).
$X_{i}$ ($1 \times R_{}$) contains $R_{}$ observed exogenous control variables with corresponding outcome-specific marginal effects given by $\beta_j$ ($R_{} \times 1$) and $\epsilon_{ij}$ is an unobserved 
% (even if $F_j$ were observed)
residual.
If we observed the components directly and had access to $K \geq L$ excludable instruments, $Z_{1i}$, we could estimate the second stage given by equation (\ref{Second_stage_true}) along with the first stage given by%
\hfill 
\begin{equation}\label{First_stage_true}
    F_{i} = Z_{i}\Gamma_{}+U_{i}
\end{equation}
via 2SLS,
where $F_{i}$ is determined by instruments $Z_{i}=[Z_{1i} \mbox{ } X_{i}]$%
%(where $X_{i}$ contains only controls that are common across $j$)
,
% $\Psi_j$ $(R \times L)$ gives the marginal association of the exogenous controls with the components,
$\Gamma_{}$ $(R_{}+K \times L)$ gives the marginal associations of the instruments with the components, $\Gamma_{k}$ gives the marginal associations of the $k$th excludeable instrument with the components, and $U_{i}$ $(1 \times L)$ represents the idiosyncratic portion of the components.%
\footnote{I  assume that there are no controls that vary across outcomes. Controls that vary with $j$ can be included into this framework if they are excluded from the first stage, as in \cite{carneiro2011estimating}. It is possible to include outcome-varying controls if the relative channels, $\theta$, through which instruments affect component treatments are assumed to be outcome-invariant, which will no longer be true by construction with multiple first stages.}
The goal of the method is to estimate the the marginal effects,
$\lambda_j$,
% and determine $L$
despite not observing $F_{i}$.
% Subscripts for individuals, $i$, on $(w,X,F,\epsilon,Z,U)$ are implied throughout.

\subsection{Decomposing Two-Stage Least Squares}\label{Model_Loop}

Because we do not observe $F_{i}$, we cannot directly estimate (\ref{Second_stage_true}) or (\ref{First_stage_true}). However, we do observe the sum of the latent factors via the composite college attendance variable,
\hfill
\begin{equation}\label{mass_def}
\begin{gathered}
D_{i} \equiv \sum_{\ell=1}^L f_{i\ell}
% x_{ij} \equiv \sum_{\ell=1}^L f_{ij\ell}
,
\end{gathered}
\end{equation}
% where $f_{ij\ell}$ $(N_j \times 1)$ is the $\ell$th component of $F_{j}$
where $F_i = [f_{i1} \mbox{ } f_{i2} \mbox{ } \dots f_{iL}]$.
% Intuitively, this constraint enforces that the composite variable is the sum of its latent components.
This presents a tractable alternative; we can estimate the observed model (in matrix notation)%
% \footnote{I think something better involves a 2nd stage that is $w_j = X_{}\beta_j +M_j \Pi_{j}+\tilde \epsilon_{j}$, where $M_j=m_j*ones_{1 \times K}$, and I calculate $\hat M_j$ with a seemingly unrelated system of first stages where each uses a single excludable instrument, $M_j = \tilde Z_j \tilde\Gamma_{} +\tilde U_j$, where $M_j$ is $N_j \times K$, $\tilde Z_j=[X \mbox{ } z_1 \mbox{ } X \mbox{ } z_2 \mbox{ } ... \mbox{ } X \mbox{ } z_K]$ is $N_j \times K(R+1)$ and 
% $\tilde\Gamma_{}$ is a quasi-diagonal $(K(R+1) \times K)$ matrix with $\Gamma_k=[\gamma_{1,k}...\gamma_{R,k} \mbox{ } \gamma_{R+1,k}]'$ along the diagonal, where $\gamma_{R+1,k}$ is the first stage coefficient on the $k$th instrument in the unique first stage that includes it.
% I think this may permit dropping the $j$ subscript and estimating a bigger SUR across jobs.
% I also think it would be good to describe (\ref{2SLS_observed}) as the reduced form system, and (\ref{Second_stage_true}) as the structural system - but I want to do so accurately, and I need to describe the parameters of this system accordingly (i.e. no $\pi_{kj}=0$).
% }
\hfill
\begin{equation}\label{2SLS_observed}
\begin{gathered}
Y_{j} = X_{k}\beta_{kj}+D\pi_{kj}+\epsilon_{kj} \\
D = Z_{}\gamma_{}+ {u}_{},
% m_{j} = X_{}\psi_j + Z_{}\gamma_{}+ u_{j},
% w_{j} = m_{j}\pi_{kj}+\epsilon_{kj} \\
% m_{j} = z_{kj}\gamma_{kj}+ u_{kj},
\end{gathered}
\end{equation}
by 2SLS,
wherein I substitute the observed composite variable, $D$ ($N \times 1$), in for the unobserved components, $F{}$ ($N \times L$).
To focus on the estimate of $\pi_{kj}$ associated with a single IV, I also include all but one of the excludable instruments as controls, defining $X_{k}=[Z_{k'} \mbox{ } X_{}]$ where $X_{}$ is $N \times R_{}$
% (noting that the controls may vary across outcomes)
and $Z_{k'}$ ($N \times K-1$) contains all excludable instruments other than a single $z_{k}$ ($N \times 1)$, such that $Z_{} = [z_{k} \mbox{ } X_{k}] $.%
\footnote{
Including all but one instrument as controls ensures that the estimate of $\pi_{kj}$ is only driven by the correlations between the excluded instrument and the latent components. Excluding other instruments from both equations would cause the estimate of $\pi_{kj}$ to reflect the correlations between other instruments and latent components via correlation between other instruments and $z_k$, making comparisons between estimates of $\pi_{kj}$ across instruments difficult. The analogous problem in the context of heterogeneous treatment effects is discussed by \cite{carneiro2011estimating} and
\cite{mogstad2021identification}.
% I think there will be something interesting to say about interpreting a Sargan J test in this context. I think the J test is invalid as a test of instrument validity.
}

In this setup, $\beta_{kj}$ ($1 \times (R_{}+K-1$)) gives the marginal effect of $X_{k}$ on $Y_{j}$, $\pi_{kj}$ gives the scalar ``effect'' of $D$ on $Y_{j}$ as determined by $z_k$, $\epsilon_{kj}$ is the idiosyncratic component of the outcome which contains the portion of $F\lambda_j$ that is not captured by $D\pi_{kj}$,
$\gamma_{}$ $((R_{}+K) \times 1)$ gives the marginal associations of the instruments with observed education, $\gamma_{k}$ gives the scalar marginal association of the $k$th excludeable instrument with the observed education, and $u$ ($N \times 1)$ is the idiosyncratic portion of observed education. Note that the instruments included in $X_{k}$ that are excludable from (\ref{Second_stage_true}) nonetheless may have nonzero coefficients within $\beta_{kj}$ because they are correlated with $F\lambda_j$, which is contained within $\epsilon_{kj}$ but is not in $\epsilon_j$.
The estimated value of $\pi_{kj}$ (as well as $\beta_{kj}$ and $\epsilon_{kj}$) varies with the excluded instrument because instruments differ in their correlations with latent components, and because each latent component affects the outcome differently.%
\footnote{An alternative framing emphasizes that the ``true'' effect of $D$ on $Y_j$ is 0 conditional on $F$. It follows that any nonzero estimate for $\pi_{kj}$ reflects omitted variable ``bias'' driven by correlation between observed schooling and unobserved components of schooling.}

Specifically,
% The structural model for wages in (\ref{Second_stage_true}) assumes no effect of composite body mass $m_j$ on wages, as well as no effect of instruments $Z_{-kj}$ on wages. This amounts to the assumptions $\pi_{kj}=0$ and $\delta_{-kj}=0$, such that comparing (\ref{Second_stage_true}) to (\ref{2SLS_observed}) shows that \hfill
% \begin{equation}\label{2SLS_bias}
% \begin{gathered}
% % w_{ij} = X_{i}\beta_{kj}+ m_{ij}\pi_{kj}+\epsilon_{ikj} \\
% % m_{ij} = X_{i}\alpha_{kj} +z_{ikj}\gamma_{kj}+ u_{ikj},
% \epsilon_{kj} = 
% F_j\lambda_j+\epsilon_j.
% \end{gathered}
% \end{equation}
% Because $X_{}$ and the excludable instruments in $Z_j$ are correlated with $F_j$ (by assumption, for $Z_{1j}$), it follows that the estimates $(\hat\beta_{kj},\hat\pi_{kj},\hat\delta_{-kj})$ will be biased in general.
% While the true parameters are invariant to the instrument, note that the estimates are instrument-specific due to differences in correlations between $z_{kj}$ and $F_j$ for each $z_{kj}$. That is, the bias is instrument-specific.
% Because I assume that $\pi_{kj}=0$ and that $Cov(z_{kj},\epsilon_j)=0$,
% Because there is no structural effect of composite body mass on wages,
% $\pi_{kj}$ must be driven by correlation between $z_{kj}$ and the unobserved $F_j\lambda_j$.%
% \footnote{Making sure only $z_{kj}$ drives $\pi_{kj}$ is the intention of including the other instruments in the second stage. If I omit them, they will affect $\pi{kj}$ through possible correlation between $z_{kj}$ and $Z_{-kj}$, and $Z_{-kj}$ and $F_j\lambda_j$.}
defining 
% $\Omega_{kj}= [\beta_{kj}' \mbox{ }  \pi_{kj}']'$, and 
$\hat{D} = Z(Z'Z)^{-1}Z'D$ and $M_X = I_N-X_{k}(X'_{k}X_{k})^{-1}X'_{k}$, we have%
\begin{equation}\label{pi_single_k_j}
\begin{split}
%   \plim_{N_j \to \infty} 
% \hat 
%   \Omega_{kj}
   \hat\pi_{kj}
    &=
    (\hat{D}'M_X{D})^{-1}\hat{D}'M_XY_j \\
    &=
    (\hat{D}'M_X{D})^{-1}\hat{D}'M_X(X_{}\beta_j+F_{}\lambda_j+\epsilon_{j}) \\
    &=
    (\hat{D}'M_X{D})^{-1}\hat{D}'M_X(F_{}\lambda_j+\epsilon_{j}) \\
    &=
    (\hat{D}'M_X{D})^{-1}\hat{D}'M_XF_{}\lambda_j+(\hat{D}'M_X{D})^{-1}\hat{D}'M_X\epsilon_{j} \\
    &=
    \theta_k \lambda_j+ {\omega}_{kj} \\    
    \end{split}
\end{equation}
where the first row is the 2SLS estimator for the ``effect'' of $D$ on $Y_j$. The second row substitutes in the definition for $Y_j$ from (\ref{Second_stage_true}). The third row substitutes $(\hat{D}'M_X{D})^{-1}\hat{D}'M_XX_{}\beta_j = 0$ by the definition of $M_X$. The fourth row separates the relationship between $z_k$ and $Y_j$ that is due to its correlation with $F$ from that which is due to its correlation with $\epsilon_j$, which may be nonzero in small samples. Finally, the fifth row extracts $\theta_k = \Gamma_k/\gamma_k=(\hat{D}'M_X\hat{D})^{-1}\hat{D}'M_XF_{}$ and defines a new error, ${\omega}_{kj} = (\hat{D}'M_X\hat{D})^{-1}\hat{D}'M_X\epsilon_{j}$. The term ${\omega}_{kj}$ converges to zero as $N$ increases if instruments are valid, so $\hat\pi_{kj}$ is a consistent estimate of $\theta_k\lambda_j$.%
\footnote{In an alternative model where unobserved factors $F_{j}$ (or controls, $X_j$) vary with $j$, $\theta_{kj}$ could also vary with $j$ (this could arise, for instance, if $j$ indexes time-periods or sub-populations). To estimate such a model with my method, it would be necessary to assume that $\theta_{kj}=\theta_k$ $\forall j$, i.e. the weights instruments place on unobserved components are common across $j$. This assumption's validity would depend on the application's instruments, outcomes, and composite treatment.\label{F_varY_j}}

Note that the weights sum to unity. Defining $\theta_k = [\theta_{k 1} \mbox{ } \theta_{k 2} \dots \theta_{k L}]$, we have \hfill
\begin{equation}\label{weights_sum_1}
\begin{split}
    \sum_{\ell=1}^L\theta_{k \ell} 
    &=
    (\hat{D}'M_X{D})^{-1}\hat{D}'M_X\sum_{\ell=1}^L f_{\ell} \\
    &=
    (\hat{D}'M_X{D})^{-1}\hat{D}'M_XD \\
    &=
    % (\hat{D}'M_X{D})^{-1}\hat{D}'M_X(\hat{D}+\hat{u}) \\
    % &=
    % (\hat{D}'M_X{D})^{-1}\hat{D}'M_X\hat{D} \\
    % &=
    1.
    \end{split}
\end{equation}
The first line follows from definitions of $\theta_{k \ell}$ and $f_{\ell}$. The second line follows from the constraint in (\ref{mass_def}).
% The third follows from the first stage in (\ref{2SLS_observed}). The fourth follows by construction given the definition of $\hat{D}$. The fifth follows from algebraic simplification.




\subsection{Identification of Component Effects}\label{Identification}

To establish identification conditions for $\theta_k$ and $\lambda_j$, I consider model (\ref{2SLS_observed}) as $N \rightarrow \infty$ separately for each instrument and each outcome, such that ${\omega}_{kj} \rightarrow 0$ for all $k$ and $j$. First, I arrange each $\pi_{kj}$ into a $K \times J$ matrix $\Pi$. Next, I define a $K\times L$ matrix $\Theta = [\theta_{1}' \mbox{ } \theta_{2}' \mbox{ } ... \mbox{ } \theta_{K}']'$, where each row of $\Theta$ gives all component weights for a single instrument.
 I  also define the $L \times J$ matrix of outcome-specific component treatment effects as $\Lambda=[\lambda_1 \mbox{ } \lambda_2 \mbox{ } ...\mbox{ } \lambda_J]$. It follows that
\begin{equation}\label{Pi_structural}
\begin{split}
% \hat
% \plim_{Nj \to \infty}\hat
\Pi = \Theta \Lambda,
\end{split}
\end{equation}
where the reduced form 2SLS estimates of $\Pi$ are thus decomposed into outcome-invariant component weights and instrument-invariant component effects.%
% \footnote{This decomposition mirrors the individual specific factors and time specific loadings in \cite{bai2009panel} and related work.}

A barrier to identification, common to factor models, is that $\Theta\Lambda = \Theta A A^{-1} \Lambda$ for an arbitrary invertible $L \times L$ matrix $A$. $A$ has $L^2$ free elements, so we require $L^2$ restrictions. To address this, I impose the normalization
\hfill
\begin{equation}\label{Normalization}
    \Theta = 
    \begin{bmatrix}
    I_L \\
    \theta_{L+1}\\
    \vdots \\
    \theta_K
    \end{bmatrix},
\end{equation}
where $I_L$ is an $L \times L$ identity matrix. The economic content of this normalization is to define the components in terms of the first $L$ instruments. For instance, if a particular instrument affects college attendance by inducing students to major in math, assigning a component to that instrument via this normalization will define it as the ``math'' type of college. Meanwhile, the associated $\lambda_j$ will give the effect of attending college with a math major on outcome $j$.

The relationships given in (\ref{weights_sum_1}), (\ref{Pi_structural}), and (\ref{Normalization}) give $K$, $KJ$, and $L^2-L$ restrictions, respectively, where the first $L$ restrictions in (\ref{weights_sum_1}) are redundant given the restrictions in (\ref{Normalization}). Meanwhile, there are $KL$ parameters in $\Theta$ and $JL$ in $\Lambda$. It follows that identification requires 
\hfill
\begin{equation*}
    L^2+KJ+K-L \geq JL+KL,
\end{equation*}
where solving for $L$ yields
\hfill
\begin{equation}\label{Identification_condition}
    L \leq (K,J+1).
\end{equation}
This expression defines the maximum number of factors that can be identified with a given number of instruments and outcomes.
Considering the simplest interesting case in which $L=2$, this requires at least two instruments and at least one outcome.
In the just-identified case, this defines $\Pi = \Lambda$ and $\Theta = I_2$. The model in this simple case is largely semantic, but still formalizes the argument that differences between $\pi_{j1}$ and $\pi_{j2}$ may be driven by differences in the latent components through which the two instruments affect the observed composite treatment.

To understand the intuition for the case with more instruments and outcomes than needed, consider the case of $L=2$, $K=3$, and $J=2$. For outcome one, the three instruments will each produce a $\hat\pi_{k,1}$. The first two IV estimates for outcome one will define components, while $\hat\pi_{3,1}$ must be either a weighted average of the first two components, or it is driven by some third component. With only one outcome, a $\Theta$ that rationalizes $\hat\pi_{3,1}$ is exactly identified as a weighted average of the first two components. However, if the $\Theta$ that rationalizes $\pi_{3,1}$ also happens to rationalize $\pi_{3,2}$, then we are able to describe the variation across 3 instruments and 2 outcomes with only 2 unobserved components. Conversely, if the value of $\Theta$ that rationalizes estimated effects across instruments in outcome one fails to do so in outcome two, then we may reject that two components can explain the data, and conclude that $L>2$ (or that treatment effect heterogeneity is responsible for the variation between IV estimates). 
% A more formal description of my procedure to identify the number of factors is in Section \ref{factor_number}.



\subsection{Estimation}
The discussion in section \ref{Model_Loop} considers a single outcome and a single instrument, but identification requires that we estimate the model using multiple outcomes and instruments as discussed in section \ref{Identification}. To do this, I leverage the analytical form of the 2SLS estimand in (\ref{pi_single_k_j}) to set $\pi_{kj} = \theta_{k}\lambda_{j}$. It follows that we can substitute $\theta_{k}\lambda_{j}$ in for $\pi_{kj}$, producing equivalent outcome equations for each excluded instrument and each outcome of the form \hfill
\begin{equation}\label{GMM_outcomes}
Y_{j} = X_{k}\beta_{kj}+D\theta_{k}\lambda_{j}+\epsilon_{kj}.
\end{equation}
 I  next leverage the assumption that $\mathbb{E}[\epsilon_{kj}'Z] = 0$, which allows us to construct moment conditions of the form \hfill
\begin{equation}\label{Moments}
\mathbb{E}[(Y_{j}-X_{k}\beta_{kj}-D\theta_{k}\lambda_{j})Z]=0.
\end{equation}
 I  then estimate the model by generalized method of moments. The estimation procedure amounts to the standard instrumental variables generalized method of moments estimator with an alternative factor-structure parameterization on treatment effects.

% Estimating system (\ref{2SLS_observed}) separately for each instrument and each outcome to collect the elements within $\Pi$ will produce consistent point estimates, but will not obtain $\Pi$'s covariance matrix, which is needed to compute standard errors for $\Theta$ and $\Lambda$. As an alternative, I estimate the seemingly-unrelated system of equations
% \hfill
% %I keep going back and forth between the next 2 versions of this
% %
% %
% %
% %Version 1
% %-------------------------------------------------------------------------------------------------------------------------------------------------
% \begin{equation}\label{SUR}
% \begin{gathered}
%     {y} = {X}{\beta}+S\Pi+\epsilon \\
%     s = {Z}\gamma+u,
%     \end{gathered}
% \end{equation}%
% where
% \begin{equation*}
% \begin{gathered}
%     y = 
%     [
%      Y_1 \mbox{ } Y_2 \dots Y_J
%     ]
%     ,
%     \quad
%     %
%       %
%     \beta = 
%     [
%      \beta_1 \mbox{ } \beta_2 \dots \beta_J
%     ]
%     ,
%     \quad
%     %
%     S = 
%     [
%      z_1\gamma_1 \mbox{ } z_2\gamma_2 \dots z_K\gamma_K
%     ]
%     ,
%     \quad
%     %
%     % \pi = 
%     % \begin{bmatrix}
%     %  \pi_1 \\
%     %  \pi_2 \\
%     %  \vdots  \\
%     %  \pi_J 
%     % \end{bmatrix}
%     % ,
%     \quad
%     %
%     \epsilon = 
%      [
%     \epsilon_1 \mbox{ } \epsilon_2 \dots \epsilon_J
%     ]
%     ,
%     % \\
%     % s = 
%     % \begin{bmatrix}
%     % s_1\\
%     % s_2\\
%     % \vdots\\
%     % s_J
%     % \end{bmatrix}
%     % ,
%     % \quad
%     % \textbf{Z} = 
%     % \begin{bmatrix}
%     % Z & 0 & \dots & 0 \\
%     % 0 & Z & \dots & 0 \\
%     % \vdots & \vdots & \ddots & \vdots \\
%     % 0 & 0 & \dots & Z
%     % \end{bmatrix} 
%     % ,
%     % \quad
%     % \gamma = 
%     % \begin{bmatrix}
%     % \gamma_1\\
%     % \gamma_2\\
%     % \vdots\\
%     % \gamma_J
%     % \end{bmatrix}
%     % ,
%     % \quad
%     % u = 
%     % \begin{bmatrix}
%     % u_1\\
%     % u_2\\
%     % \vdots\\
%     % u_J
%     % \end{bmatrix}
%     % ,
%     \end{gathered}
% \end{equation*}
% where $S$ contains all excluded instruments' contributions to $s$ from the first stage.%
% %
% %
% %
% %Version 2
% %-------------------------------------------------------------------------------------------------------------------------------------------------
% % \begin{equation}\label{SUR}
% % \begin{gathered}
% %     {y} = \mathbf{X}{\beta}+\mathbf{D}\Pi^c+\epsilon \\
% %     s = {Z}\gamma+u,
% %     \end{gathered}
% % \end{equation}%
% % where
% % \begin{equation*}
% % \begin{gathered}
% %     y = 
% %     \begin{bmatrix}
% %      Y_1 \\
% %      Y_2 \\
% %      \vdots  \\
% %      Y_J 
% %     \end{bmatrix}
% %     ,
% %     \quad
% %     %
% %     \mathbf{X} = 
% %     \begin{bmatrix}
% %     X & 0 & \dots & 0 \\
% %     0 & X & \dots & 0 \\
% %     \vdots & \vdots & \ddots & \vdots \\
% %     0 & 0 & \dots & X
% %     \end{bmatrix} 
% %     ,
% %     \quad
% %     %
% %     \beta = 
% %     \begin{bmatrix}
% %      \beta_1 \\
% %      \beta_2 \\
% %      \vdots  \\
% %      \beta_J 
% %     \end{bmatrix}
% %     ,
% %     \\
% %     %
% %     \mathbf{D} = 
% %     \begin{bmatrix}
% %     S & 0 & \dots & 0 \\
% %     0 & S & \dots & 0 \\
% %     \vdots & \vdots & \ddots & \vdots \\
% %     0 & 0 & \dots & S
% %     \end{bmatrix} 
% %     ,
% %     \quad
% %     S = 
% %     \begin{bmatrix}
% %     z_1'\gamma_1 \\
% %     z_2'\gamma_2 \\
% %     \vdots \\
% %     z_K'\gamma_K
% %     \end{bmatrix}'
% %     ,
% %     \quad
% %     %
% %     % \pi = 
% %     % \begin{bmatrix}
% %     %  \pi_1 \\
% %     %  \pi_2 \\
% %     %  \vdots  \\
% %     %  \pi_J 
% %     % \end{bmatrix}
% %     % ,
% %     \quad
% %     %
% %     \epsilon = 
% %     \begin{bmatrix}
% %     \epsilon_1\\
% %     \epsilon_2\\
% %     \vdots\\
% %     \epsilon_J
% %     \end{bmatrix},
% %     % \\
% %     % s = 
% %     % \begin{bmatrix}
% %     % s_1\\
% %     % s_2\\
% %     % \vdots\\
% %     % s_J
% %     % \end{bmatrix}
% %     % ,
% %     % \quad
% %     % \textbf{Z} = 
% %     % \begin{bmatrix}
% %     % Z & 0 & \dots & 0 \\
% %     % 0 & Z & \dots & 0 \\
% %     % \vdots & \vdots & \ddots & \vdots \\
% %     % 0 & 0 & \dots & Z
% %     % \end{bmatrix} 
% %     % ,
% %     % \quad
% %     % \gamma = 
% %     % \begin{bmatrix}
% %     % \gamma_1\\
% %     % \gamma_2\\
% %     % \vdots\\
% %     % \gamma_J
% %     % \end{bmatrix}
% %     % ,
% %     % \quad
% %     % u = 
% %     % \begin{bmatrix}
% %     % u_1\\
% %     % u_2\\
% %     % \vdots\\
% %     % u_J
% %     % \end{bmatrix}
% %     % ,
% %     \end{gathered}
% % \end{equation*}
% % where $\Pi^c$ is the $KJ \times 1$ column vectorization of $\Pi$.%
% %
% %
% %
% %
% %
% \footnote{This seemingly-unrelated regressions set-up can be generalized to the case where treatments or controls vary with $j$, with the elements of $y$ stacked vertically and with block diagonal matrices $\mathbf{X}$ and $\mathbf{D}$, with blocks containing elements $X_j$ and $S_j$, respectively, for all $j$. Such a set-up requires an additional assumption as described in footnote \ref{F_varY_j}.}

% Estimating the model this way will obtain estimates of all elements of $\Pi$ simultaneously. Because the elements in ${D}$ are linear in $z_{k}$ for all $k$, the inclusion of all elements of $S$ in the second stage effectively includes all other instruments as controls when considering the effect associated with each single instrument, as recommended by \cite{carneiro2011estimating} and \cite{mogstad2021identification}. This procedure also estimates only $J$ seemingly unrelated systems, rather than $KJ$ (as would be needed if performing the system analog to (\ref{2SLS_observed})). This procedure also estimates the covariance of $\Pi$ without requiring post-estimation calculations. 

% I estimate $\Theta$ and $\Lambda$ by choosing $(\hat \Theta, \hat \Lambda)$ to minimize $\hat \Pi-\hat \Theta \hat \Lambda$ while imposing the restrictions in (\ref{weights_sum_1}) and (\ref{Normalization}).
% I will describe the estimation more thoroughly in a future version of the paper.



% \subsection{Determining the Number of Factors}\label{factor_number}
% This section is very preliminary.
% \cite{su2017time} have a method for doing this that I will likely apply, but I have not yet done so.

% The intuition for determining the number of factors is as follows. I want to explain all of the variation in $\Pi$ with my factor model (at odds with many factor models used in economics). Hence, if I have $K>L$ instruments and have correctly chosen $L$, it should be the case that $\Pi = \Theta \Lambda$ despite being apparently overidentified. I estimate $\hat\Theta \hat\Lambda$ by minimizing $\hat\Omega = \hat\Theta \hat\Lambda - \hat \Pi$, where $\hat\Omega$ will be nonzero if $L$ factors are insufficient to completely explain the data, or due to sampling error in $\hat\Omega$. So in essence, the number of factors can be determined by estimating the model using $ L^*=1,2,...,K$ sequentially, and testing the hypothesis that $\hat\Omega = 0$. If I fail to reject the null, then I conclude that $L=L^*$.

% Another avenue toward identifying the number of factors is that because $\Pi$ is a linear combination of effects of unobserved factors ($\Lambda$), it should be the case that $L=rank(\Pi)$. In practice, it is likely that $\hat \Pi$ will be full rank due to sampling noise, even if $K>L$. It follows that a hypothesis test for the rank of $\Pi$ will identify $L$.

% An alternative approach when considering the number of factors to acknowledge that there may be an arbitrarily large number of component treatments (considering, for instance, the number of finely-defined topics a person might study during their years of education), each of which may have different effects on outcomes. Approaching the model from this perspective suggests accepting ex ante that $L>>K$. Here, nonetheless, I can determine the amount of variation in $\hat{\Pi}$ that is explained by $\hat{\Theta}\hat{\Lambda}$ for $L=1,\dots,K$. This allows inference regarding the number of component treatments that are particularly important for driving outcomes.

% \subsection{Testing Instrument Strength}

% This section is very preliminary. 

% The thrust of this section is that in the context of my model, an instrument might significantly increase one type of education while reducing a different type. An example of such an instrument is one that causes students to choose a particular major in college over another. Such instruments may be strong in the unobserved first stage in (\ref{First_stage_true}), but weak in the observed first stage in (\ref{2SLS_observed}).

% Such instruments produce problems in the heterogeneous treatment effects framework, where the reduced form effect of the instrument on the outcome might be large if component treatments have very different effects, while the observed first stage would be weak. One likely conclusion in such a setting is that such an instrument must be invalid. In my framework, a strong observed first stage is sufficient but not necessary for a strong unobserved first stage. It follows that my model likely has implications for weak instrument tests and corrections, but I are still in the early stages of such inquiries.

==> Sections/Results/Results_v1.tex <==
\section{Results}

 I  begin by showing results for two stage least squares estimates for each year, excluding each instrument and including the others as controls. These results are in Table \ref{tab:TSLS}, and shown graphically in Figure \ref{fig:TSLS}. I note that my results are broadly in line with the literature, especially directing the reader to wage returns around age 30, as this is approximately the age typically targeted by other papers on returns to college that look at a single snapshot in the lifecycle. I also observe substantial variation both between instruments and across time, with returns as driven by local earnings yielding the most extreme results. This is suggestive that the type of education sought by individuals who are sensitive to local earnings produces high wage returns, which is reasonable considering these individuals have revealed themselves in some sense to be particularly money-motivated.

 I  also show the estimated effects from the unobserved treatment heterogeneity model of two unobserved components of college on earnings over a sample of the lifecycle below. I define the first component in terms of local earnings at age 17 and the other in terms of local tuition at age 17. The unobserved hneterogeneity results naturally inherit similarities from the 2SLS results, but allow for instruments that may not satisfy Net Monotonicity to nonetheless contribute to identification of treatment effects. A main advantage of including the additional instrument that may not positively weight all component treatments is that it contributes to efficiency in the estimation, making the unobserved treatment heterogeneity estimates substantially more precise than the just-identified IV.


\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Just-Identified 2SLS Estimates of Lifecycle Returns to College, by IV}
\label{tab:TSLS}
\begin{tabular}{l*{7}{c}}
\hline
\input{Figures_Tables/TSLS_table}
\hline
\hline
\end{tabular}
\begin{minipage}{1\linewidth}
\smallskip
\footnotesize
\emph{Notes:} Two-stage least squares estimates of the effects of college attendance on log wages for white men in the NLSY79. Age-specific estimates obtained excluding a single instrument and including all others as controls along with the other control variables listed in Table \ref{tab:descriptives}. College returns are annualized by dividing the college attendance coefficient by four. Robust standard errors in parentheses. 
\end{minipage}
\end{table}

\begin{figure}[hbtp!]
\centering
\includegraphics[width=.8\linewidth]{Figures_Tables/TSLS_graph_no_CI.png}
\begin{minipage}{1\linewidth}
\caption{2SLS Estimates of Lifecycle Wage Returns to College}
\label{fig:TSLS}
\smallskip
\footnotesize
\emph{Notes:} This graph depicts just identified 2SLS point estimates of the effect of college attendance on lifecycle log wages for each excluded instrument listed. See Table \ref{tab:TSLS} for point estimates and standard errors.
\end{minipage}
\end{figure}




\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{GMM Estimates of Lifecycle Returns to Unobserved College Components}
\label{tab:UTH}
\begin{tabular}{l*{7}{c}}
\hline
\input{Figures_Tables/UTH_table}
\end{tabular}
\begin{minipage}{1\linewidth}
\smallskip
\footnotesize
\emph{Notes:} Two-step generalized method of moments estimates of the effects of unobserved types of college attendance on log wages for white men in the NLSY79. Component-defining instruments have weights normalized to 1 on respective components. College returns are annualized by dividing the college component effects by four. Robust standard errors in parentheses. 
\end{minipage}
\end{table}

\begin{figure}[hbtp!]
\centering
\includegraphics[width=.8\linewidth]{Figures_Tables/UTH_graph_no_CI.png}
\begin{minipage}{1\linewidth}
\caption{GMM Estimates of Lifecycle Wage Returns to Unobserved College Components}
\label{fig:Lambda_hat}
\smallskip
\footnotesize
\emph{Notes:} This graph depicts GMM point estimates of the effects of unobserved college components on lifecycle log wages for components defined in terms of listed instruments. See Table \ref{tab:UTH} for point estimates and standard errors.
\end{minipage}
\end{figure}

There are three main ways to interpret results such as those I have described from my unobserved heterogeneity model. The first, most ambitious way, is to take a strong stance on the types of college education that are induced by each instrument, such that I can strictly define component effects identified by each IV as in \cite{kline2016evaluating}. If I were comfortable saying, for instance, that local earnings cause students to major in math and local tuition costs cause students to major in art, I would interpret Figure \ref{fig:Lambda_hat} as showing the returns to math and art over the lifecycle. This seems quite extreme given the instruments I have on hand for this application, but may be appropriate for other treatments or with other instruments.

A weaker approach to interpretation is to consider more broadly the channels through which instruments might work, so as to get a sense of the likely drivers of treatment effect heterogeneity. For instance, I note that individuals induced to attend college by local earnings must have some (at least indirect) information about and interest in wage differentials across career choices. Such individuals may find earnings differentials between different education choices particularly salient, and may be relative well-informed about them. Students for whom college distance looms large may prioritize nonpecuniary benefits of college over pecuniary returns, as pecuniary transit costs are relatively small compared to pecuniary returns to college. I could infer, then, that the local earnings instrument identifies the effect of high pecuniary-return college, and the nearby college instrument identifies the effect of high amenity-return college.

A still weaker approach to interpretation of results is to leave clarification on exact channels through which instruments affect outcomes to future work that gathers more data on treatment variations. In this framework, the unobserved heterogeneity estimates give insight into the scope and scale of treatment heterogeneity. This would serve as a guide to future research that endeavors to obtain finer data on treatments in an effort to parse out effects of component treatments. Additionally, instruments that are suspected of violating Condition \ref{net_monotonicity} can still be included so as to contribute to efficiency, without taking a strong stance on the channels through which each instrument affects outcomes.
With this approach to interpretation, the assumption that some instruments assumed to satisfy Condition \ref{net_monotonicity} work only through particular component treatments is a normalization that fails to pin down a single economically relevant treatment, but does prevent more suspicious instruments from contaminating results.

==> Sections/Theory/Theory.tex <==
I  work with a potential outcomes framework similar to that used by \cite{imbens1994identification}, with reference as well to \cite{rubin1974estimating,rubin1990comment}, \cite{heckman1990varieties}, and \cite{angrist1991sources}. The main innovation in my paper is to model an observed composite treatment, $D_i$, as being composed of $L$ unobserved component treatments $\{D_{i1},D_{i2},...D_{iL}\}$ such that $D_i=\sum_{\ell=1}^LD_{i\ell}$. I consider binary component and composite treatments for simplicity of exposition in this section.%
\footnote{It follows that each individual will either have $D_{i\ell}$=0 for all $\ell$ or $D_{i\ell}=0$ for all $\ell\neq m$ and $D_{im}=1$.}
 I  define $Y_i(0)$ as the value of the outcome in the absence of treatment, which is observed when the individual selects none of the available component treatments. I next define $Y_i(\ell)$, for $\ell=1,2,...,L$ as the value of the outcome when $D_{i1}=1$, $D_{i2}=1$, ..., or $D_{iL}=1$, respectively.
% Finally, I define $Y_i(1)$ as the value of the outcome for person $i$ in the presence of their most-preferred component treatment. 

 We  observe $Y_i(0)$ for individuals that do not select treatment, but not those that do, as is standard in the potential outcomes framework. However, with unobserved treatment heterogeneity, $D_i=1$ is not sufficient to determine the value of $D_{i\ell}$, other than to bound $\ell$ at $\ell>0$. It follows that not only do we not observe $Y_i(\ell)|D_i=0$ for any $i$ or $\ell>0$, but we also do not observe $Y_i(\ell)|D_{im}=1$ for any $i$ for any combination of $\ell$ and $m$.%
\footnote{More precisely, we do observe $Y_i(\ell)$ for individuals who choose component treatment $\ell$, but I do not know the $\ell$ for which we are observing $Y_i(\ell)$.}
This muddling of potential outcomes for treated individuals is the central empirical challenge I address in this paper. Not only is the single composite treatment effect not observed for any individuals, it not well-defined. We instead are left with multiple component treatment effects, $Y_i(\ell)-Y_i(0)$, which can be differenced to define unobserved treatment switching effects, $Y_i(\ell)-Y_i(\ell')$ for all $\ell \neq \ell '$.

In the language of the Rubin \citeyearpar{rubin1974estimating} causal model, unobserved treatment heterogeneity constitutes a violation of the stable unit treatment value assumption (SUTVA). In randomized controlled trials, random assignment to treatment ensures that $\mathbb{E}[Y_i(\ell)|D_{i\ell}=1] = \mathbb{E}[Y_i(\ell)|D_{im}=1]$ for all $\ell$ and $m$, including the cases where $\ell=0$ or $m=0$. Experimental control efforts are intended to ensure that $D_i=D_{i\ell}$ for a given $\ell$ for all individuals in an observed treatment arm. In other words, the administration of the treatment is explicitly designed to hold equal between treated individuals all variations that are expected to substantively alter the nature of the treatment.\footnote{Even well-designed experiments differ in this respect. Variation in subtle priming from the outward affect or word choices of research staff administering a medical treatment might not complicate treatment effect identification for treatments of physical ailments but may do so for treatments of psychological ailments.} The control of the trial ensures identification of treatment effects that are entirely driven by a single component treatment, while the randomization ensures that the effects can be estimated via comparisons of treated and untreated individuals.

\subsection{Problems and Solutions for Instrumental Variables}

It is common for researchers to use instrumental variables to estimate the effects of treatments, especially when randomized controlled trials are infeasible or when random policy variation is assumed to affect outcomes through known channels. I consider a vector of instrumental variables, $Z_i$, within a subset $\mathcal{Z}$ of $\mathbb{R}^K$, where $K$ gives the number of instruments. I define an instrument as a variable that satisfies the following conditions. 
First, it is independent of $Y(0)$ and $Y(\ell)$ for all $\ell=1,...,L$. Second, it is correlated with the composite treatment $D_i$, which implies correlation with at least one unobserved component treatment in $\{D_{i\ell}\}_{\ell=1}^L$. 
For any vector value $z$ within $\mathcal{Z}$, I define $D_{i\ell}(z)$ to be the value of the $\ell$th component treatment for $i$ if the value of $Z_i$ is equal to $z$. We observe $(Y_i,D_i,Z_i)$ for a random sample of a population of interest. The key distinction in this discussion from that in \cite{imbens1994identification} is that different values of the instrument not only shift people into and out of the composite treatment, but they also determine which component treatment the individual selects. Formally, I define an instrument according to the following condition:

\begin{condition}[Existence of Instruments]\label{existence_of_instruments}
Let $Z$ be a vector of random variables such that (i) for all $z\in \mathcal{Z}$ the $(2L+1)$-tuple  $(Y(0),Y(1),...,Y(L),D_{i1}(z),...,D_{iL}(z))$ is jointly independent of $Z_i$, and (ii) $P(z)=\mathbb{E}[D_i|Z_i=z]$ is a nontrivial function of $z$.
\end{condition}
The difference between this condition and that given by \cite{imbens1994identification} is the presence of multiple treatments $(D_{i1}(z),...,D_{iL}(z))$ and potential outcomes $(Y(0),Y(1),...,Y(L))$. Part $(ii)$ is testable in applications, and further implies that $P_\ell(z)=\mathbb{E}[D_{i\ell}|Z_i=z]$ is a nontrivial function of $z$ for at least some $\ell$ in $\ell=1,2,...,L$. The effects of the instrument on individual component treatments are not testable because the component treatments are unobserved.

To demonstrate the problems that unobserved treatment effect heterogeneity presents for identification of average treatment effects, I compare expected outcomes at two distinct values of the instrument, $\mathbb{E}[Y_i|Z_i=z]$ and $\mathbb{E}[Y_i|Z_i=z']$. Taking differences, we have \hfill
\begin{equation*}
\begin{split}
    \mathbb{E}[Y_i&|Z_i=z] - \mathbb{E}[Y_i|Z_i=z'] \\
    =
    &\mathbb{E}[\sum_{\ell=1}^L D_{i\ell}(z)Y_i(\ell)+(1-\sum_{\ell=1}^L D_{i\ell}(z))Y_i(0)|Z_i=z] \\
    -&\mathbb{E}[\sum_{\ell=1}^L D_{i\ell}(z')Y_i(\ell)+(1-\sum_{\ell=1}^L D_{i\ell}(z'))Y_i(0)|Z_i=z'].
    \end{split}
\end{equation*}
%You are here
Condition 1 implies that this is equal to
\begin{equation}\label{Nonparametic_Reduced_Form_Decomposition}
\begin{split}
    \sum_{\ell=1}^L
    \mathbb{E}
    &\Big[(D_{i\ell}(z)-D_{i\ell}(z'))(Y_i(\ell)-Y_i(0)) \Big] \\
    = 
    % &
    &\sum_{\ell=1}^L \Pr[D_{i\ell}(z)-D_{i\ell}(z')=1]\mathbb{E}[Y_i(\ell)-Y_i(0)|D_{i\ell}(z)-D_{i\ell}(z')=1] \\
    - 
    &\sum_{\ell=1}^L \Pr[D_{i\ell}(z)-D_{i\ell}(z')=-1]\mathbb{E}[Y_i(\ell)-Y_i(0)|D_{i\ell}(z)-D_{i\ell}(z')=-1].
    %
    % \mathbb{E}\Big[(D_{i\ell}(z)-D_{i\ell}(z'))(Y_i(\ell)-Y_i(0)) \Big],
    \end{split}
\end{equation}
% \begin{split}
%     &\mathbb{E}[(D_{i1}(z)-D_{i1}(z'))(Y_i(1,0)-Y_i(0,0))+(D_{i2}(z)-D_{i2}(z'))(Y_i(0,1)-Y_i(0,0))] \\
%     =
%     % &(\Pr(D_{i1}(z)-D_{i1}(z')=1)-\Pr(D_{i1}(z)-D_{i1}(z')=-1))\mathbb{E}[(Y_i(1,0)-Y_i(0,0))] \\
%     % &\mathbb{E}[D_{i1}(z)-D_{i1}(z')]\mathbb{E}[(Y_i(1,0)-Y_i(0,0))] \\
%     &(P_1(z)-P_1(z'))\mathbb{E}[(Y_i(1,0)-Y_i(0,0))] \\
%     % &\mathbb{E}[D_{i1}(z)]\mathbb{E}[(Y_i(1,0)-Y_i(0,0))]-\mathbb{E}[D_{i1}(z')]\mathbb{E}[(Y_i(1,0)-Y_i(0,0))] \\
%     +
%     % &(\Pr(D_{i2}(z)-D_{i2}(z')=1)-\Pr(D_{i2}(z)-D_{i2}(z')=-1))\mathbb{E}[(Y_i(0,1)-Y_i(0,0))].
%     % &\mathbb{E}[D_{i2}(z)-D_{i2}(z')]\mathbb{E}[(Y_i(0,1)-Y_i(0,0))]
%     &(P_2(z)-P_2(z'))\mathbb{E}[(Y_i(0,1)-Y_i(0,0))],
%     \end{split}
% \end{equation}
This expression suggests two potential problems for average treatment effect identification. The first, described in detail by \cite{imbens1994identification}, occurs with treatment effect heterogeneity when $\mathbb{E}[Y_i(\ell)-Y_i(0)|D_{i\ell}(z)-D_{i\ell}(z')=1] \neq \mathbb{E}[Y_i(\ell)-Y_i(0)|D_{i\ell}(z)-D_{i\ell}(z')=-1]$. The additional problem highlighted here occurs with treatment heterogeneity when $\mathbb{E}[Y_i(\ell)-Y_i(0)|D_{i\ell}(z)-D_{i\ell}(z')=a] \neq \mathbb{E}[Y_i(\ell')-Y_i(0)|D_{i\ell'}(z)-D_{i\ell'}(z')=a]$ for $a=-1,1$.

To more clearly illustrate this new problem, consider the case of homogeneous treatment effects across individuals for each unobserved component treatment. This reduces equation (\ref{Nonparametic_Reduced_Form_Decomposition}) to
\hfill
\begin{equation}\label{Homogeneous_Nonparametic_Reduced_Form_Decomposition}
\begin{split}
    \sum_{\ell=1}^L\mathbb{E}\Big[(D_{i\ell}(z)-D_{i\ell}(z'))(Y_i(\ell)-Y_i(0)) \Big]
    = 
    % &
    &\sum_{\ell=1}^L(P_{\ell}(z)-P_{\ell}(z'))\lambda_\ell \\
     =
     & \sum_{\ell=1}^L I(P_\ell(z) \geq P_\ell(z'))(P_{\ell}(z)-P_{\ell}(z'))\lambda_\ell \\
     -
     & \sum_{\ell=1}^L I(P_\ell(z) \leq P_\ell(z'))(P_{\ell}(z')-P_{\ell}(z))\lambda_\ell
    \end{split}
\end{equation}
where $P_\ell(z) = \mathbb{E}[D_{i\ell}|Z_i=z]$ gives the probability of component treatment $\ell$ at instrument value $z$, $\lambda_\ell$ gives the homogeneous treatment effect for component treatment $\ell$, and $I(\cdot)$ is an indicator function that takes a value of unity if its argument is true and zero otherwise.
Even with this simplification, unobserved treatment heterogeneity leaves room for variation in identified treatment effects for the composite treatment, $D_i$, when using different instrumental variables (or different shifts in the value of a single instrument). 

To see this, consider the case of two component treatments, where the second component treatment effect is double that of the first, and the change in the value of the instrument shifts equal numbers of individuals from nontreatment and the second component treatment into the first component treatment. Formally, this entails
\hfill
\begin{equation*}
    \lambda_2 = 2\lambda_1
\end{equation*}
and \hfill
\begin{equation*}
\begin{gathered}
    P_1(z)-P_1(z') = -2(P_2(z)-P_2(z')).
    \end{gathered}
\end{equation*}
Substituting these expressions into equation (\ref{Homogeneous_Nonparametic_Reduced_Form_Decomposition}) yields a difference in outcomes of zero regardless of the strength of the first stage or the magnitudes or signs of the component treatment effects. Amplifying the disparities in component treatments' effects or responses to the instrument further can produce negative IV estimands even when all underlying component treatment effects are positive, and vice versa. 
Intuitively, if some individuals respond to the instrument by changing their treatment type to or from an extreme version of the treatment, the type they select out of will be weighted negatively and the type they select into will be weighted positively, even though their observed composite treatment status has not changed.%
\footnote{For example, consider a randomized STEM-specific college scholarship. We might expect such a scholarship to induce some individuals to switch from non-college to STEM-college and some to switch from non-STEM-college to STEM-college. If STEM majors have relatively high returns, using this policy as an instrument for college attendance will overstate returns to college.}

To identify an effect of the composite treatment that is a positively-weighted average of the effects of component treatments, I present the following assumption on instruments in addition to those described in Condition \ref{existence_of_instruments}. %
%There is a very general condition, which does the following
%1. Switchers are replaced by compliers with the same returns (doesn't have to be same treatment, just a treatment for compliers that has same effect on compliers as the treatment effect of the treatment switchers had on switchers (changes in outcomes are cancelled out). 
%a. No switchers (i.e. monotonicity for all component treatments) is a special case of this.
%b. Homogeneous treatment effects with no *net* switching is a special case of this.
% You identify Y(ell)-Y(0)|D_iell(z)>D_iell(z')
%Even more important - I can have defiers, I just need people with the same returns as the defiers to be compliers. There are 2 basic ways to do this:
%1. For the group of defiers for instrument comparison z and z', the same group of people are compliers for instrument comparison z'' and z'''. If P(z'')-P(z''')>=P(z)-P(z'), the net shift of this sort of person doing this type of treatment is positive, so there are no net defiers across all values of the instrument. This is the insight behind MTW partial monotonicity.
%2. You can also have no net defiers across a single instrument comparison, if there are compliers for that comparison who happen to have the same treatment effects as the defiers.
% So, broadly, you can either cancel out the defiers of type A with compliers of type B for a given instrument comparison if A's return to the treatment they switch out of is equal to B's return to the treatment they switch into, or you can cancel out defiers of type A at a particular instrument comparison with defiers of type A at a different instrument comparison.
% \begin{condition}[Net Monotonicity]\label{net_monotonicity}
% For all $z,z'\in \mathcal{Z}$, either (i) $D_{i\ell}(z)-D_{i\ell}(z') = \mbox{sgn}(P(z)-P(z'))$, (ii) $D_{i\ell}(z)-D_{i\ell}(z') = 0$, or (iii) $\exists $ $j$ such that $D_{j \ell}(z)-D_{j \ell}(z')=\mbox{sgn}(P(z)-P(z'))$, $Y_j(\ell)-Y_j(0)=Y_i(\ell)-Y_i(0)$, and $i$ and $j$ form a unique pairing, for all $i$ and for all $\ell$.
% \end{condition}
%Define people who share i's treatment effect, then say 
\begin{condition}[Net Monotonicity]\label{net_monotonicity}
For all $z,z'\in \mathcal{Z}$, either (i) $D_{i\ell}(z)-D_{i\ell}(z') = \mbox{sgn}(P(z)-P(z'))$, (ii) $D_{i\ell}(z)-D_{i\ell}(z') = 0$ for all $i$ and all $\ell$, or (iii) $Pr(D_{j\ell}(z)-D_{j\ell}(z') = \mbox{sgn}(P(z)-P(z'))|Y_j(\ell)-Y_j(0)=Y_i(\ell)-Y_i(0)) \geq
Pr(D_{j\ell}(z)-D_{j\ell}(z') = -\mbox{sgn}(P(z)-P(z'))|Y_j(\ell)-Y_j(0)=Y_i(\ell)-Y_i(0))$ for all $\ell$.
\end{condition}
% \begin{condition}[Net Monotonicity]\label{net_monotonicity}
% For all $z,z'\in \mathcal{Z}$, either (i) $D_{i\ell}(z)-D_{i\ell}(z') = \mbox{sgn}(P(z)-P(z'))$, (ii) $D_{i\ell}(z)-D_{i\ell}(z') = 0$, or (iii) there exists a set $\mathcal{I}_{i\ell} \subseteq \mathcal{I}$ such that all $j \in \mathcal{I}_{i\ell}$ have $Y_j(\ell)-Y_j(0)=Y_i(\ell)-Y_i(0)$ and $Pr(D_{j\ell}(z)-D_{j\ell}(z') = \mbox{sgn}(P(z)-P(z'))|j \in \mathcal{I}_{i\ell}) \geq Pr(D_{i\ell}(z)-D_{i\ell}(z') = \mbox{sgn}(P(z)-P(z')))$     P_\ell(z') and a $z'' \in \mathcal{Z}$ such that $D_{j m}(z)-D_{j m}(z'')=\mbox{sgn}(P(z)-P(z'))$ and for some $m$ in $1,2,...,L$, for all $i$. 
% \end{condition}
% \begin{condition}[Net Monotonicity]\label{net_monotonicity}
% For all $z,z'\in \mathcal{Z}$, either (i) $D_{i\ell}(z)-D_{i\ell}(z') = \mbox{sgn}(P(z)-P(z'))$, (ii) $D_{i\ell}(z)-D_{i\ell}(z') = 0$, or (iii) there exists a $j$ and a $z'' \in \mathcal{Z}$ such that $D_{j m}(z)-D_{j m}(z'')=\mbox{sgn}(P(z)-P(z'))$ and $Y_j(m)-Y_j(0)=Y_i(\ell)-Y_i(0)$ for some $m$ in $1,2,...,L$, for all $i$. 
% \end{condition}
% \begin{condition}[Treatment Response Homogeneity]\label{net_monotonicity}
% For all $z,z'\in \mathcal{Z}$, either \\ $\mathbb{E}[D_{i\ell}(z)]\geq \mathbb{E}[D_{i\ell}(z')]$ for all $\ell$, or $\mathbb{E}[D_{i\ell}(z)]\leq \mathbb{E}[D_{i\ell}(z')]$ for all $\ell$.
% \end{condition}
Cases (i) and (ii) correspond to the monotonicity condition described by \cite{imbens1994identification}, extended to the current setting with multiple unobserved treatments. \cite{kline2016evaluating} describe a similar condition that restricts changes in the treatment decision to a single observed component treatment in the presence of multiple observed component treatments, while \cite{hull2018isolateing} describes a similar condition that restricts changes in treatment decision from one of multiple observed untreated states to a single observed component treatment. The relevant distinction in this paper is that even when (i) and (ii) hold for all individuals, my Condition \ref{net_monotonicity} still permits multiple unobserved types of treatment, wherein identified treatment effects are not only weighted averages of treatment effects for particular groups of individuals, but also for particular component treatments.

To better discuss case (iii), I adapt the language of \cite{angrist1996identification} to describe groups of individuals with respect to their component treatment statuses for different instrument comparisons. A component $\ell$ always-taker chooses component treatment $\ell$ regardless of their value for $Z_i$. A component $\ell$ never-taker never chooses component treatment $\ell$ regardless of their value for $Z_i$. Always takers for any component $\ell$ are necessarily never-takers for all other component treatments, as well as the untreated state. Component $\ell$ compliers at instrument comparison $z,z'$ have $D_{i\ell}(z)-D_{i\ell}(z') = \mbox{sgn}(P(z)-P(z'))$. Finally, component $\ell$ defiers at instrument comparison $z,z'$ have $D_{i\ell}(z)-D_{i\ell}(z') = -\mbox{sgn}(P(z)-P(z'))$.

Case (iii) of Condition \ref{net_monotonicity} essentially allows for defiers for any component as long as there are compliers for that component to cancel them out. When a subset of compliers cancel out defiers, the local treatment effect estimated at the instrument comparison will be driven by the residual subset of compliers that do not cancel out defiers. 
% A graphical illustration of the residual compliers is provided in Figure \ref{fig:residual_compliers} (placeholder for a link to a figure that shows Panel A, a frequency distribution over treatment effects, where the complier frequency is higher at all values of the support, and Panel B, the frequency distribution of compliers minus defiers at each point in the support).

To define this set of residual compliers more formally, I define the set of defiers for component treatment $\ell$ at $z,z'$ as $\mathcal{I}_{\ell}^{D;z,z'}$ and the set of compliers for component $\ell$  as $\mathcal{I}^{C;z,z'}_{\ell}$. I then partition the data such that $i=1,\dots,N_{D1} \in \mathcal{I}^{D;z,z'}_{1}, i=N_{D1}+1,\dots,N_{D1}+N_{C1} \in \mathcal{I}^{C;z,z'}_{1}, \dots , i=\sum_{\ell=1}^{L-1}N_{D\ell}+N_{C\ell}+1,\dots,\sum_{\ell=1}^{L-1}N_{D\ell}+N_{C\ell}+N_{DL} \in \mathcal{I}^{D;z,z'}_{L}$,
$i=\sum_{\ell=1}^{L-1}N_{D\ell}+N_{C\ell}+1,\dots,\sum_{\ell=1}^{L}N_{D\ell}+N_{C\ell} \in \mathcal{I}^{C;z,z'}_{L}$, where $N_{D\ell}$ is the number of defiers for component treatment $\ell$ and $N_{C\ell}$ is the number of compliers for component treatment $\ell$. In words, I order individuals such that defiers for component treatment 1 are first, followed by compliers for component treatment 1, then defiers for component 2, and so on (with always-takers and never-takers for all component treatments coming last). Within the set $\mathcal{I}^{D;z,z'}_{\ell}$ for each $\ell$, I order individuals such that $Y_{i}(\ell)-Y_{i}(0) \leq Y_{i+1}(\ell)-Y_{i+1}(0)$ for all $i \in \mathcal{I}^{D;z,z'}_{\ell}$. Within the set $\mathcal{I}^{C;z,z'}_{\ell}$, I order individuals such that $\sum_{i=N_{-\ell}+N_{D\ell}+1}^{N_{-\ell}+2N_{D\ell}}|(Y_{i}(\ell)-Y_{i}(0)) - (Y_{i-N_{D\ell}}(\ell)-Y_{i-N_{D\ell}}(0))|$ is minimized, where I define $N_{-\ell} = \sum_{m=1}^{\ell-1}N_{Dm}+N_{Cm}$. I define a residual complier for component treatment $\ell$ as an $i \in \mathcal{I}_{\ell}^{RC}$ for whom $i > N_{-\ell}+2N_{D\ell}$. In words, this ordering pairs each defier for component treatment $\ell$ with a complier for component treatment $\ell$ at the same position within the order of compliers, such that compliers that are not paired with a defier have relatively high values of the index $i$. Condition \ref{net_monotonicity} ensures that the minimum of $\sum_{i=N_{-\ell}+N_{D\ell}+1}^{N_{-\ell}+2N_{D\ell}}|(Y_{i}(\ell)-Y_{i}(0)) - (Y_{i-N_{D\ell}}(\ell)-Y_{i-N_{D\ell}}(0))|=0$ such that each defier-complier pair have equal treatment effects.

Other similar sufficient conditions exist for identification of positively-weighted local average component treatment effects. One is the existence of a value of the instrument $z$ such that $P(z)=0$ or $P(z)=1$, such that all comparisons of $z,z'\in \mathcal{Z}$ only include compliers for all component treatments, as discussed in the homogeneous treatment setting by \cite{heckman1990varieties} and \cite{angrist1991sources}.\footnote{The particular value of restricting individuals to these two cases is one advantage of randomized controlled trials.} An intuitively similar condition allows for defiers at some instrument comparisons as long as a sufficient mass of individuals with the same treatment effect are compliers at other instrument comparisons, as described in \cite{mogstad2021identification}.\footnote{The tests described in \cite{mogstad2021identification} to determine whether there are sufficient compliers at well-behaved instrument comparisons to cancel out noncompliers at poorly-behaved instrument comparisons are not immediately applicable to settings with unobserved treatment heterogeneity.} I concentrate on my Condition \ref{net_monotonicity} because cases (i) and (ii) are analogous to the commonly-invoked \cite{imbens1994identification} monotonicity condition, while case (iii) simplifies to the following under component treatment effect homogeneity:
\begin{condition}[Homogeneous Treatment Effects Net Monotonicity]\label{homogeneous_effects_net_monotonicity}
    (i) $Y_i(\ell)-Y_i(0) = \lambda_\ell$ for all  $i$ and (ii) for all $z,z'\in \mathcal{Z}$,  either
    $P_{\ell}(z)\geq P_{\ell}(z') $
    for all $\ell$,
    or $P_{\ell}(z)\leq P_{\ell}(z')$  for all  $\ell$.
\end{condition}
\noindent This condition preserves the logic of the IA monotonicity condition with the modification that the relevant compliers for instrument comparisons are component treatments rather than individuals.



We  can identify an average treatment effect of the composite treatment using instrumental variables by dividing the difference in outcomes at different values of instruments expressed in (\ref{Nonparametic_Reduced_Form_Decomposition}) by the net difference in the share of the population that chooses the composite treatment. Condition 2 ensures that this average treatment effect is a positively weighted average of underlying component treatment effects for a subset of the population of interest. Formally, I provide the following result:
\begin{thm}
    If Conditions \textnormal{\ref{existence_of_instruments}} and \textnormal{\ref{net_monotonicity}} hold, the average treatment effect defined by 
    \begin{equation*}
    \pi_{z,z'} = 
    \sum_{\ell=1}^L
    \theta_\ell
    \mathbb{E}
    \Big[
    Y_i(\ell)-Y_i(0)
    \Big|
    % D_{i\ell}(z) - D_{i\ell}(z') = sgn(P(z)-P(z')),
    i \in \mathcal{I}_\ell^{RC;z,z'}
    \Big]
    \end{equation*}
    % \begin{equation*}
    % \begin{split}
    % \frac{\mathbb{E}[Y_i|Z_i=z] - \mathbb{E}[Y_i|Z_i=z']}
    % {P(z)-P(z')}\\
    % &= 
    % \sum_{\ell=1}^L
    % \frac{
    % P_\ell(z)-P_\ell(z')
    % \lambda_\ell
    % }
    % {P(z)-P(z')
    % }
    % .
    % \end{split}
    % \end{equation*}
    % \begin{equation*}
    % \begin{split}
    % \pi_{z,z'} &= 
    % \frac{\mathbb{E}[Y_i|Z_i=z] - \mathbb{E}[Y_i|Z_i=z']}
    % {P(z)-P(z')}\\
    % &= 
    % \sum_{\ell=1}^L
    % \frac{
    % P_\ell(z)-P_\ell(z')
    % \lambda_\ell
    % }
    % {P(z)-P(z')}
    % .
    % \end{split}
    % \end{equation*}
    is identified from the joint distribution of $(Y,D,Z)$ and $\theta_\ell \in [0,1]$ for all $\ell=1,2,...,L$ for all $z,z'\in\mathcal{Z}$ such that $\mathbb{E}[Y_i|Z_i=z]$ and $\mathbb{E}[Y_i|Z_i=z']$ are finite and $P(z)\neq P(z')$, with  $\theta_\ell$ given by
    \begin{equation*}
        \theta_\ell = 
        \frac{
    P_\ell(z)-P_\ell(z')
    }
    {P(z)-P(z')
    }.
    \end{equation*}
\end{thm}

\begin{proof}
Let Condition \ref{existence_of_instruments} be satisfied. It follows that equation (\ref{Nonparametic_Reduced_Form_Decomposition}) holds. Using the sets defined above, this expression is equivalent to
\begin{equation*}
\begin{split}
    \mathbb{E}[Y_i&|Z_i=z] - \mathbb{E}[Y_i|Z_i=z'] \\
    = 
    % &
    &\sum_{\ell=1}^L 
    \Pr(i\in \mathcal{I}_\ell^{RC;z,z'})\mathbb{E}[Y_i(\ell)-Y_i(0)|i\in \mathcal{I}_\ell^{RC;z,z'}] \\
    +
    &\sum_{\ell=1}^L \Pr(i\in \mathcal{I}_\ell^C,i\not\in \mathcal{I}_\ell^{RC;z,z'})\mathbb{E}[Y_i(\ell)-Y_i(0)|i\in \mathcal{I}_\ell^C,i\not\in \mathcal{I}_\ell^{RC;z,z'}] \\
    - 
    &\sum_{\ell=1}^L \Pr(i\in \mathcal{I}_\ell^{D;z,z'})\mathbb{E}[Y_i(\ell)-Y_i(0)|i\in \mathcal{I}_\ell^{D;z,z'}].
    %
    % \mathbb{E}\Big[(D_{i\ell}(z)-D_{i\ell}(z'))(Y_i(\ell)-Y_i(0)) \Big],
    \end{split}
\end{equation*}
Let Condition \ref{net_monotonicity} be satisfied as well. It follows from the definitions of the sets $\mathcal{I}_\ell^{D;z,z'}$, $\mathcal{I}_\ell^{C;z,z'}$, and $\mathcal{I}_\ell^{RC;z,z'}$  that the last two lines of the above expression cancel out, yielding
\begin{equation*}
\begin{split}
    \mathbb{E}[Y_i&|Z_i=z] - \mathbb{E}[Y_i|Z_i=z'] \\
    = 
    % &
    &\sum_{\ell=1}^L 
    \Pr(i\in \mathcal{I}_\ell^{RC;z,z'})\mathbb{E}[Y_i(\ell)-Y_i(0)|i\in \mathcal{I}_\ell^{RC;z,z'}].
    \end{split}
\end{equation*}
Given that $D_{i\ell}(z)-D_{i\ell}(z') \neq 0$ iff $i\in \mathcal{I}_\ell^{C;z,z'}$ or $i\in \mathcal{I}_\ell^{D;z,z'}$, it follows that $\Pr(i\in \mathcal{I}_\ell^{RC;z,z'}) = P_\ell(z)-P_\ell(z')$. Making this substitution and multiplying the right-hand side of the equation by $(P(z)-P(z'))/(P(z)-P(z'))$ gives
\begin{equation*}
\begin{split}
    \mathbb{E}[Y_i&|Z_i=z] - \mathbb{E}[Y_i|Z_i=z'] \\
    = 
    % &
    &
    (P(z)-P(z'))\sum_{\ell=1}^L 
    \frac{
    P_\ell(z)-P_\ell(z')
    }
    {
    P(z)-P(z')
    }
    \mathbb{E}[Y_i(\ell)-Y_i(0)|i\in \mathcal{I}_\ell^{RC;z,z'}].
    \end{split}
\end{equation*}
Dividing each side of the equation by $(P(z)-P(z'))$ shows that the local component average treatment effect $\pi_{z,z'}$ is identified in terms of moments of the distribution of $(Y,D,Z)$.
\end{proof}





% Case (iii) allows for component treatment defiers so long as they are cancelled out by compliers who share their treatment effects. The case in which defiers at some instrument comparisons are compliers at other instrument comparisons is a multi-treatment extension of the partial monotonicity assumption described by \cite{mogstad2021identification}. I also allow for the case in which different groups of individuals at the same (or different) instrument comparisons happen to have the same treatment effects as the defiers for the component treatment they move out of. This can occur in three main ways, two of which are relatively straightforward. The first is the case in which an individual switches between component treatments that share the same idiosyncatic effect for them, in which case they are a complier for one component treatment that cancels out a defier for another (themselves). The second is the case of homogeneous component treatment effects, in which all that is necessary is that all aggregate changes in component treatment shares match the sign of the change in composite treatment.\footnote{The homogeneous component treatment effect version of Condition 2 can be constructed by removing (iii) and substituting $P$ in for $D_i$ throughout the statement of the condition.} Finally, it is possible that complier individuals at the same or different instrument value comparisons happen to have the same treatment effects at their chosen component treatments as the defiers had at the component treatments for which they are defiers.

Figure \ref{fig:Net_monotonicity_illustration} shows a graphical illustration of the decision setting. The horizontal axes give a latent utility index for the composite treatment, such that the composite treatment is chosen if $V_i\geq0$. The vertical axes give a relative preference for two component treatments, such that treatment 1 is chosen if $V_{1i} \geq 0$ and $V_i\geq0$, and treatment 2 is chosen if $V_{11} < 0$ and $V_i\geq0$. The ovals drawn in each figure contain uniform joint distributions of individuals' preferences for treatments. Each panel shows a different instrument comparison assumed to satisfy Condition \ref{existence_of_instruments}. The instrument shift in panel A satisfies Condition \ref{net_monotonicity} without any individual defiers for any component treatment. The shift in panel B satisfies Condition \ref{net_monotonicity} under a homogeneous component treatment effects assumption, while the shift in panel C does not. 
% In each case, Condition \ref{net_monotonicity} may be satisfied if the treatment effects of compliers happen to match those of defiers for the component treatment for which they are a defier.%
%\footnote{Note that if the two component treatments have the same effects for each individual, Condition \ref{net_monotonicity} will be trivially satisfied for each instrument shown.}




%\newgeometry{margin=1cm} % modify this if you need even more space
%\begin{landscape}
\begin{SidewaysFigure}

    \centering
    \begin{subfigure}[t]{0.4\textwidth}
    \raggedright
        Panel A
        \begin{center}
        \resizebox{\textwidth}{!}{
\begin{tikzpicture}
\node[label=below:{$D=0$} ]   () at (-3.0, -2) {};
\node[label=above:{$D=0$} ]   () at (-3.0, 2) {};
\node[label=below:{$D_{2}=1$} ]   () at (3.0, -2) {};
\node[label=above:{$D_{1}=1$} ]   () at (3.0, 2) {};
\node[label=below:{$V$} ]   () at (3.5, 0) {};
\node[label=right:{$V_1$} ]   () at (0, 2.5) {};
\node[label=above:z']   () at (.6, -.7) {};
\node[label=above:z]   () at (1.3, -.7) {};

\draw [-{Latex[round]}] (0,0) -- (0,3);
\draw [-{Latex[round]}] (0,0) -- (0,-3);
\draw[white, thick] (-4,0) -- (0,0); %To center
\draw [-{Latex[round]}] (0,0) -- (4,0);
\draw [-{Latex[round]}] (0,0) -- (-4,0);
\draw[rotate=45][gray, dashed] (-1,0) ellipse (60pt and 30pt);
\draw [-{Latex[round]}] (0,0) -- (0,-3);
\draw[rotate=45] (-.5,-.5) ellipse (60pt and 30pt);
\draw [-{Latex[round]}] (.7,-.6) -- (1.4,-.6);
\end{tikzpicture}
}
\end{center}
\end{subfigure}
\hspace{0.05\textwidth}%
%
%
%
%
    \begin{subfigure}[t]{0.4\textwidth}
    \raggedright
        Panel B
        \begin{center}
        \resizebox{\textwidth}{!}{
\begin{tikzpicture}
\node[label=below:{$D=0$} ]   () at (-3.0, -2) {};
\node[label=above:{$D=0$} ]   () at (-3.0, 2) {};
\node[label=below:{$D_{2}=1$} ]   () at (3.0, -2) {};
\node[label=above:{$D_{1}=1$} ]   () at (3.0, 2) {};
\node[label=below:{$V$} ]   () at (3.5, 0) {};
\node[label=right:{$V_1$} ]   () at (0, 2.5) {};
\node[label=below:z']   () at (.8, .8) {};
\node[label=below:z]   () at (1.5, 1.5) {};

\draw [-{Latex[round]}] (0,0) -- (0,3);
\draw [-{Latex[round]}] (0,0) -- (0,-3);
\draw[white, thick] (-4,0) -- (0,0); %To center
\draw [-{Latex[round]}] (0,0) -- (4,0);
\draw [-{Latex[round]}] (0,0) -- (-4,0);
\draw[rotate=45][gray, dashed] (-1,0) ellipse (60pt and 30pt);
\draw [-{Latex[round]}] (0,0) -- (0,-3);
\draw[rotate=45] (0,0) ellipse (60pt and 30pt);
\draw [-{Latex[round]}] (.8,.8) -- (1.5,1.5);
\end{tikzpicture}
}
\end{center}
\end{subfigure}
\hspace{0.05\textwidth}%
%
%
%
    \begin{subfigure}[t]{0.4\textwidth}
    \raggedright
        Panel C
        \begin{center}
        \resizebox{\textwidth}{!}{
\begin{tikzpicture}
\node[label=below:{$D=0$} ]   () at (-3.0, -2) {};
\node[label=above:{$D=0$} ]   () at (-3.0, 2) {};
\node[label=below:{$D_{2}=1$} ]   () at (3.0, -2) {};
\node[label=above:{$D_{1}=1$} ]   () at (3.0, 2) {};
\node[label=below:{$V$} ]   () at (3.5, 0) {};
\node[label=right:{$V_1$} ]   () at (0, 2.5) {};
\node[label=below:z']   () at (0.2,-1.4) {};
\node[label=below:z]   () at (.8,-2.1) {};

\draw [-{Latex[round]}] (0,0) -- (0,3);
\draw [-{Latex[round]}] (0,0) -- (0,-3);
\draw[white, thick] (-4,0) -- (0,0); %To center
\draw [-{Latex[round]}] (0,0) -- (4,0);
\draw [-{Latex[round]}] (0,0) -- (-4,0);
\draw[rotate=45][gray, dashed] (-1,0) ellipse (60pt and 30pt);
\draw [-{Latex[round]}] (0,0) -- (0,-3);
\draw[rotate=45] (-1,-1) ellipse (60pt and 30pt);
\draw [-{Latex[round]}] (0.1,-1.4) -- (.8,-2.1);
\end{tikzpicture}
}
\end{center}
\end{subfigure}
\caption{Instrument Comparisons with Two Unobserved Component Treatments}
\label{fig:Net_monotonicity_illustration}
   \begin{minipage}{1\linewidth}
\smallskip
\footnotesize
\emph{Notes:} For composite treatment preference $V$ and relative preference for component treatment 1 $V_1$, each panel shows a different instrument comparison. Panel A depicts an instrument comparison where individuals' preference for treatment increases, but there is no effect on the composition of treatment (no defiers). Panel B shows a comparison where more individuals choose each type of treatment at $z$ than at $z'$, but there are compositional changes in the individuals who choose each component treatment. If component treatment effects are homogeneous, the situation in Panel B will satisfy my Net Monotonicity condition. Panel C depicts an instrument comparison where the aggregate composition of treatment shifts in response to the treatment. Net monotonicity will only hold in this setting if the idiosyncratic treatment effects of compliers cancel out the treatment effects for the group of people who shift from component treatment 1 to component treatment 2, for instance if component 1 and component 2 have identical treatment effects for defiers.
\end{minipage}
\end{SidewaysFigure}

%\end{landscape}
%\restoregeometry

The assumption that no individuals switch their preferred version of treatment in response to instruments may be strong in many settings, even those in which Imbens and Angrists' monotonicity assumption is uncontroversial. For instance, an instrument that reduces costs for college may produce income effects, which may cause some students to obtain leisure by choosing lower-earnings majors%
%\citep{leslie turner}
. It may seem similarly strong to assume that there happen to be compliers that exactly cancel out defiers as I describe in case (iii) of Condition \ref{net_monotonicity}. However, if treatment composition shifts are small relative to net shifts in treatment, the number of compliers who are available to cancel out defiers will be relatively large. If the defier treatment effect distribution is encompassed by the support of the complier treatment effect distribution, Condition \ref{net_monotonicity} will be satisfied if compliers sufficiently outnumber defiers. The economic content of such an assumption is that instrumental variables cause shifts in observed composite treatments that are large relative to unobserved component treatment shifts, which seems likely to be satisfied in many settings where a strict person-specific component treatment monotonicity condition would be violated.




% To fix ideas, I take the opportunity to describe a policy-relevant example of an instrument that. Consider a policy that gives students a large college scholarship that is contingent on the student pursing humanities coursework. Suppose further that the wage return to the humanities type of college education is half that of the wage return to non-humanities college (saying nothing about non-wage returns). It is very likely that such a policy, if well-publicized, would have a strong first stage, reflecting its effect on shifting individuals into college. Furthermore, it is likely that such a policy would also induce some students who planned on pursuing non-humanities coursework to instead pursue humanities course work. Using the implementation of this policy as an instrumental variable for the return to college, therefore, would then result in estimates of the return to college that would be below those for both humanities college education and non-humanities college education.

==> Sections/Theory/Theory_v2.tex <==
%
%
%
%
\section{2SLS with Unobserved Treatment Heterogeneity}
In this section, I will describe conditions under which standard IV methods identify meaningful average effects of treatments with unobserved heterogeneity. 
In the context of the \cite{rubin1974estimating} causal model (RCM), unobserved treatment heterogeneity constitutes a violation of the Stable Unit Treatment Value Assumption, which requires there to be only one version of each treatment. 
I will start by presenting the problem using RCM language and notation.
Next, I will present sufficient conditions for treatment effect identification in the case where treatments are heterogeneous and their effects are homogeneous, wherein unobserved defier and complier treatments will play similar roles to those of defier and complier individuals in the more familiar case of homogeneous treatments with heterogeneous effects.
Afterward, I will allow for both unobserved treatment heterogeneity and treatment effect heterogeneity with a strict monotonicity assumption related to those of \cite{imbens1994identification} and \cite{heckman2018unordered}.
I close the section by relaxing this monotonicity assumption for cases when treatments and their effects are heterogeneous by applying the insights of \cite{de2017tolerating} to allow for compliers (for some version of treatment) to cancel out defiers (for some version of the treatment) who share their treatment effects.


\subsection{Potential Outcomes with Unobserved Treatment Heterogeneity}
I  work with a potential outcomes framework similar to that used by \cite{angrist1996identification}, with reference as well to \cite{rubin1974estimating,rubin1990comment}, \cite{heckman1990varieties}, \cite{angrist1991sources}, and \cite{imbens1994identification}. 
Beginning with the case of a single instrument, I denote the $N$-dimensional vector of values of the instrumental variable for all $N$ individuals as $\mathbf{Z}$, with $Z_i$ the particular value for individual $i$.
The main innovation of this paper concerns an observed composite treatment for individual $i$, $D_i(\mathbf{Z})$, that is composed of $L$ unobserved mutually exclusive component treatments such that $D_i(\mathbf{Z})=\sum_{\ell=1}^LD_{i\ell}(\mathbf{Z})$, with the vector $\mathbf{D}_i(\mathbf{Z}) = (D_{i1}(\mathbf{Z}),D_{i2}(\mathbf{Z}),...D_{iL}(\mathbf{Z}))$ denoting $i$'s treatment status for each version of the treatment and the $N \times L$ matrix $\mathbf{D}(\mathbf{Z})$ denoting component treatment statuses for all individuals as a function of the instrument vector.
I consider binary component and composite treatments for simplicity of exposition in this section.%
% \footnote{It follows that each individual will either have $D_{i\ell}$=0 for all $\ell$ or $D_{i\ell}=0$ for all $\ell\neq m$ and $D_{im}=1$.}


I define $Y_i(\mathbf{Z},\mathbf{D})$ as the value of an outcome taking as given instruments and unobserved component treatments, with $N$-dimensional vector $\mathbf{Y}(\mathbf{Z},\mathbf{D})$ denoting outcomes for all individuals.
In the context of my application, $\mathbf{Y}(\mathbf{Z},\mathbf{D})$ gives wages for all individuals for a particular year as a function of the value of the instrument (such as local tuition at age 17) and their unobserved treatment statuses (such as their chosen majors or course-effort allocations in college).
Though I have modeled unobserved treatments as binary, allowing for arbitrarily many versions implicitly allows for any combination or level of treatment by encoding each as a mutually exclusive alternative treatment.

Modeling an outcome from individual $i$ as a function of the entire matrix of treatment types and instruments for all individuals presents problems for estimating treatment effects, as datasets do not contain alternate values of $(\mathbf{Z},\mathbf{D})$. 
The immediate goal is to define individual-level treatment effects for unobserved component treatments that are not functions of instruments or other individuals' treatments.
I begin by assuming that the observed value of the instrument $Z_i$ is sufficient to describe the instrument assignment and that the $L$ unobserved treatments are sufficient to describe all unobserved heterogeneity in treatment
\begin{condition}[Stable Unit Unobserved Treatment Value Assumption]\label{SUUTVA}
\hfill 

a. If $Z_i = Z_i'$, then $D_{i\ell}(\mathbf{Z})= D_{i\ell}(\mathbf{Z}')$.

b. If $Z_i = Z_i'$ and $D_{i\ell} = D_{i\ell}'$, then $Y_i(\mathbf{Z},\mathbf{D}) = Y_i(\mathbf{Z}',\mathbf{D}')$.
\end{condition}

Part a. of this condition rules out unmodeled heterogeneity in the instrument, as in the case of $Z_i$ represents an binary indicator for receipt of a college scholarship, where $Z_i$ represents an unmodeled STEM-major-contingent college scholarship and $Z_i'$ represents an unmodeled non-contingent scholarship.
Part b. also rules out unmodeled variation in treatment, as in the case where $D_{i\ell}$ occurs in a state of the world where individual $i$ chooses major $\ell$ and works hard, and $D_{i\ell}'$ occurs in a state of the world where individual $i$ chooses major $\ell$ and slacks off.
This condition has bite for instruments, where it must be the case that instrumental variables are defined sufficiently finely.
With respect to treatments, it is trivially satisfied by allowing for arbitrarily many varieties of treatment.%
\footnote{The commonly discussed case of spillovers is covered by treatment heterogeneity, where individual $j$ (not) receiving treatment while $i$ receives (no) treatment is modeled as a particular version of the treatment received by $i$.}







We  observe $Y_i(0)$ for individuals that do not select treatment, but not those that do, as is standard in the potential outcomes framework. However, with unobserved treatment heterogeneity, $D_i=1$ is not sufficient to determine the value of $D_{i\ell}$, other than to bound $\ell$ at $\ell>0$. It follows that not only do we not observe $Y_i(\ell)|D_i=0$ for any $i$ or $\ell>0$, but we also do not observe $Y_i(\ell)|D_{im}=1$ for any $i$ for any combination of $\ell$ and $m$.%
\footnote{More precisely, we do observe $Y_i(\ell)$ for individuals who choose component treatment $\ell$, but I do not know the $\ell$ for which we are observing $Y_i(\ell)$.}
This muddling of potential outcomes for treated individuals is the central empirical challenge I address in this paper. Not only is the single composite treatment effect not observed for any individuals, it not well-defined. We instead are left with multiple component treatment effects, $Y_i(\ell)-Y_i(0)$, which can be differenced to define unobserved treatment switching effects, $Y_i(\ell)-Y_i(\ell')$ for all $\ell \neq \ell '$.









I  define $Y_i(0)$ as the value of the outcome in the absence of treatment, which is observed when the individual selects none of the available component treatments. I next define $Y_i(\ell)$, for $\ell=1,2,...,L$ as the value of the outcome when $D_{i1}=1$, $D_{i2}=1$, ..., or $D_{iL}=1$, respectively.
% Finally, I define $Y_i(1)$ as the value of the outcome for person $i$ in the presence of their most-preferred component treatment. 

 We  observe $Y_i(0)$ for individuals that do not select treatment, but not those that do, as is standard in the potential outcomes framework. However, with unobserved treatment heterogeneity, $D_i=1$ is not sufficient to determine the value of $D_{i\ell}$, other than to bound $\ell$ at $\ell>0$. It follows that not only do we not observe $Y_i(\ell)|D_i=0$ for any $i$ or $\ell>0$, but we also do not observe $Y_i(\ell)|D_{im}=1$ for any $i$ for any combination of $\ell$ and $m$.%
\footnote{More precisely, we do observe $Y_i(\ell)$ for individuals who choose component treatment $\ell$, but I do not know the $\ell$ for which we are observing $Y_i(\ell)$.}
This muddling of potential outcomes for treated individuals is the central empirical challenge I address in this paper. Not only is the single composite treatment effect not observed for any individuals, it not well-defined. We instead are left with multiple component treatment effects, $Y_i(\ell)-Y_i(0)$, which can be differenced to define unobserved treatment switching effects, $Y_i(\ell)-Y_i(\ell')$ for all $\ell \neq \ell '$.

In the language of the Rubin \citeyearpar{rubin1974estimating} causal model, unobserved treatment heterogeneity constitutes a violation of the stable unit treatment value assumption (SUTVA). In randomized controlled trials, random assignment to treatment ensures that $\mathbb{E}[Y_i(\ell)|D_{i\ell}=1] = \mathbb{E}[Y_i(\ell)|D_{im}=1]$ for all $\ell$ and $m$, including the cases where $\ell=0$ or $m=0$. Experimental control efforts are intended to ensure that $D_i=D_{i\ell}$ for a given $\ell$ for all individuals in an observed treatment arm. In other words, the administration of the treatment is explicitly designed to hold equal between treated individuals all variations that are expected to substantively alter the nature of the treatment.\footnote{Even well-designed experiments differ in this respect. Variation in subtle priming from the outward affect or word choices of research staff administering a medical treatment might not complicate treatment effect identification for treatments of physical ailments but may do so for treatments of psychological ailments.} The control of the trial ensures identification of treatment effects that are entirely driven by a single component treatment, while the randomization ensures that the effects can be estimated via comparisons of treated and untreated individuals.

\subsection{Problems and Solutions for Instrumental Variables}

It is common for researchers to use instrumental variables to estimate the effects of treatments, especially when randomized controlled trials are infeasible or when random policy variation is assumed to affect outcomes through known channels. I consider a vector of instrumental variables, $Z_i$, within a subset $\mathcal{Z}$ of $\mathbb{R}^K$, where $K$ gives the number of instruments. I define an instrument as a variable that satisfies the following conditions. 
First, it is independent of $Y(0)$ and $Y(\ell)$ for all $\ell=1,...,L$. Second, it is correlated with the composite treatment $D_i$, which implies correlation with at least one unobserved component treatment in $\{D_{i\ell}\}_{\ell=1}^L$. 
For any vector value $z$ within $\mathcal{Z}$, I define $D_{i\ell}(z)$ to be the value of the $\ell$th component treatment for $i$ if the value of $Z_i$ is equal to $z$. We observe $(Y_i,D_i,Z_i)$ for a random sample of a population of interest. The key distinction in this discussion from that in \cite{imbens1994identification} is that different values of the instrument not only shift people into and out of the composite treatment, but they also determine which component treatment the individual selects. Formally, I define an instrument according to the following condition:

\begin{condition}[Existence of Instruments]\label{existence_of_instruments}
Let $Z$ be a vector of random variables such that (i) for all $z\in \mathcal{Z}$ the $(2L+1)$-tuple  $(Y(0),Y(1),...,Y(L),D_{i1}(z),...,D_{iL}(z))$ is jointly independent of $Z_i$, and (ii) $P(z)=\mathbb{E}[D_i|Z_i=z]$ is a nontrivial function of $z$.
\end{condition}
The difference between this condition and that given by \cite{imbens1994identification} is the presence of multiple treatments $(D_{i1}(z),...,D_{iL}(z))$ and potential outcomes $(Y(0),Y(1),...,Y(L))$. Part $(ii)$ is testable in applications, and further implies that $P_\ell(z)=\mathbb{E}[D_{i\ell}|Z_i=z]$ is a nontrivial function of $z$ for at least some $\ell$ in $\ell=1,2,...,L$. The effects of the instrument on individual component treatments are not testable because the component treatments are unobserved.

To demonstrate the problems that unobserved treatment effect heterogeneity presents for identification of average treatment effects, I compare expected outcomes at two distinct values of the instrument, $\mathbb{E}[Y_i|Z_i=z]$ and $\mathbb{E}[Y_i|Z_i=z']$. Taking differences, we have \hfill
\begin{equation*}
\begin{split}
    \mathbb{E}[Y_i&|Z_i=z] - \mathbb{E}[Y_i|Z_i=z'] \\
    =
    &\mathbb{E}[\sum_{\ell=1}^L D_{i\ell}(z)Y_i(\ell)+(1-\sum_{\ell=1}^L D_{i\ell}(z))Y_i(0)|Z_i=z] \\
    -&\mathbb{E}[\sum_{\ell=1}^L D_{i\ell}(z')Y_i(\ell)+(1-\sum_{\ell=1}^L D_{i\ell}(z'))Y_i(0)|Z_i=z'].
    \end{split}
\end{equation*}
%You are here
Condition 1 implies that this is equal to
\begin{equation}\label{Nonparametic_Reduced_Form_Decomposition}
\begin{split}
    \sum_{\ell=1}^L
    \mathbb{E}
    &\Big[(D_{i\ell}(z)-D_{i\ell}(z'))(Y_i(\ell)-Y_i(0)) \Big] \\
    = 
    % &
    &\sum_{\ell=1}^L \Pr[D_{i\ell}(z)-D_{i\ell}(z')=1]\mathbb{E}[Y_i(\ell)-Y_i(0)|D_{i\ell}(z)-D_{i\ell}(z')=1] \\
    - 
    &\sum_{\ell=1}^L \Pr[D_{i\ell}(z)-D_{i\ell}(z')=-1]\mathbb{E}[Y_i(\ell)-Y_i(0)|D_{i\ell}(z)-D_{i\ell}(z')=-1].
    %
    % \mathbb{E}\Big[(D_{i\ell}(z)-D_{i\ell}(z'))(Y_i(\ell)-Y_i(0)) \Big],
    \end{split}
\end{equation}
% \begin{split}
%     &\mathbb{E}[(D_{i1}(z)-D_{i1}(z'))(Y_i(1,0)-Y_i(0,0))+(D_{i2}(z)-D_{i2}(z'))(Y_i(0,1)-Y_i(0,0))] \\
%     =
%     % &(\Pr(D_{i1}(z)-D_{i1}(z')=1)-\Pr(D_{i1}(z)-D_{i1}(z')=-1))\mathbb{E}[(Y_i(1,0)-Y_i(0,0))] \\
%     % &\mathbb{E}[D_{i1}(z)-D_{i1}(z')]\mathbb{E}[(Y_i(1,0)-Y_i(0,0))] \\
%     &(P_1(z)-P_1(z'))\mathbb{E}[(Y_i(1,0)-Y_i(0,0))] \\
%     % &\mathbb{E}[D_{i1}(z)]\mathbb{E}[(Y_i(1,0)-Y_i(0,0))]-\mathbb{E}[D_{i1}(z')]\mathbb{E}[(Y_i(1,0)-Y_i(0,0))] \\
%     +
%     % &(\Pr(D_{i2}(z)-D_{i2}(z')=1)-\Pr(D_{i2}(z)-D_{i2}(z')=-1))\mathbb{E}[(Y_i(0,1)-Y_i(0,0))].
%     % &\mathbb{E}[D_{i2}(z)-D_{i2}(z')]\mathbb{E}[(Y_i(0,1)-Y_i(0,0))]
%     &(P_2(z)-P_2(z'))\mathbb{E}[(Y_i(0,1)-Y_i(0,0))],
%     \end{split}
% \end{equation}
This expression suggests two potential problems for average treatment effect identification. The first, described in detail by \cite{imbens1994identification}, occurs with treatment effect heterogeneity when $\mathbb{E}[Y_i(\ell)-Y_i(0)|D_{i\ell}(z)-D_{i\ell}(z')=1] \neq \mathbb{E}[Y_i(\ell)-Y_i(0)|D_{i\ell}(z)-D_{i\ell}(z')=-1]$. The additional problem highlighted here occurs with treatment heterogeneity when $\mathbb{E}[Y_i(\ell)-Y_i(0)|D_{i\ell}(z)-D_{i\ell}(z')=a] \neq \mathbb{E}[Y_i(\ell')-Y_i(0)|D_{i\ell'}(z)-D_{i\ell'}(z')=a]$ for $a=-1,1$.

To more clearly illustrate this new problem, consider the case of homogeneous treatment effects across individuals for each unobserved component treatment. This reduces equation (\ref{Nonparametic_Reduced_Form_Decomposition}) to
\hfill
\begin{equation}\label{Homogeneous_Nonparametic_Reduced_Form_Decomposition}
\begin{split}
    \sum_{\ell=1}^L\mathbb{E}\Big[(D_{i\ell}(z)-D_{i\ell}(z'))(Y_i(\ell)-Y_i(0)) \Big]
    = 
    % &
    &\sum_{\ell=1}^L(P_{\ell}(z)-P_{\ell}(z'))\lambda_\ell \\
     =
     & \sum_{\ell=1}^L I(P_\ell(z) \geq P_\ell(z'))(P_{\ell}(z)-P_{\ell}(z'))\lambda_\ell \\
     -
     & \sum_{\ell=1}^L I(P_\ell(z) \leq P_\ell(z'))(P_{\ell}(z')-P_{\ell}(z))\lambda_\ell
    \end{split}
\end{equation}
where $P_\ell(z) = \mathbb{E}[D_{i\ell}|Z_i=z]$ gives the probability of component treatment $\ell$ at instrument value $z$, $\lambda_\ell$ gives the homogeneous treatment effect for component treatment $\ell$, and $I(\cdot)$ is an indicator function that takes a value of unity if its argument is true and zero otherwise.
Even with this simplification, unobserved treatment heterogeneity leaves room for variation in identified treatment effects for the composite treatment, $D_i$, when using different instrumental variables (or different shifts in the value of a single instrument). 

To see this, consider the case of two component treatments, where the second component treatment effect is double that of the first, and the change in the value of the instrument shifts equal numbers of individuals from nontreatment and the second component treatment into the first component treatment. Formally, this entails
\hfill
\begin{equation*}
    \lambda_2 = 2\lambda_1
\end{equation*}
and \hfill
\begin{equation*}
\begin{gathered}
    P_1(z)-P_1(z') = -2(P_2(z)-P_2(z')).
    \end{gathered}
\end{equation*}
Substituting these expressions into equation (\ref{Homogeneous_Nonparametic_Reduced_Form_Decomposition}) yields a difference in outcomes of zero regardless of the strength of the first stage or the magnitudes or signs of the component treatment effects. Amplifying the disparities in component treatments' effects or responses to the instrument further can produce negative IV estimands even when all underlying component treatment effects are positive, and vice versa. 
Intuitively, if some individuals respond to the instrument by changing their treatment type to or from an extreme version of the treatment, the type they select out of will be weighted negatively and the type they select into will be weighted positively, even though their observed composite treatment status has not changed.%
\footnote{For example, consider a randomized STEM-specific college scholarship. We might expect such a scholarship to induce some individuals to switch from non-college to STEM-college and some to switch from non-STEM-college to STEM-college. If STEM majors have relatively high returns, using this policy as an instrument for college attendance will overstate returns to college.}

To identify an effect of the composite treatment that is a positively-weighted average of the effects of component treatments, I present the following assumption on instruments in addition to those described in Condition \ref{existence_of_instruments}. %
%There is a very general condition, which does the following
%1. Switchers are replaced by compliers with the same returns (doesn't have to be same treatment, just a treatment for compliers that has same effect on compliers as the treatment effect of the treatment switchers had on switchers (changes in outcomes are cancelled out). 
%a. No switchers (i.e. monotonicity for all component treatments) is a special case of this.
%b. Homogeneous treatment effects with no *net* switching is a special case of this.
% You identify Y(ell)-Y(0)|D_iell(z)>D_iell(z')
%Even more important - I can have defiers, I just need people with the same returns as the defiers to be compliers. There are 2 basic ways to do this:
%1. For the group of defiers for instrument comparison z and z', the same group of people are compliers for instrument comparison z'' and z'''. If P(z'')-P(z''')>=P(z)-P(z'), the net shift of this sort of person doing this type of treatment is positive, so there are no net defiers across all values of the instrument. This is the insight behind MTW partial monotonicity.
%2. You can also have no net defiers across a single instrument comparison, if there are compliers for that comparison who happen to have the same treatment effects as the defiers.
% So, broadly, you can either cancel out the defiers of type A with compliers of type B for a given instrument comparison if A's return to the treatment they switch out of is equal to B's return to the treatment they switch into, or you can cancel out defiers of type A at a particular instrument comparison with defiers of type A at a different instrument comparison.
% \begin{condition}[Net Monotonicity]\label{net_monotonicity}
% For all $z,z'\in \mathcal{Z}$, either (i) $D_{i\ell}(z)-D_{i\ell}(z') = \mbox{sgn}(P(z)-P(z'))$, (ii) $D_{i\ell}(z)-D_{i\ell}(z') = 0$, or (iii) $\exists $ $j$ such that $D_{j \ell}(z)-D_{j \ell}(z')=\mbox{sgn}(P(z)-P(z'))$, $Y_j(\ell)-Y_j(0)=Y_i(\ell)-Y_i(0)$, and $i$ and $j$ form a unique pairing, for all $i$ and for all $\ell$.
% \end{condition}
%Define people who share i's treatment effect, then say 
\begin{condition}[Net Monotonicity]\label{net_monotonicity}
For all $z,z'\in \mathcal{Z}$, either (i) $D_{i\ell}(z)-D_{i\ell}(z') = \mbox{sgn}(P(z)-P(z'))$, (ii) $D_{i\ell}(z)-D_{i\ell}(z') = 0$ for all $i$ and all $\ell$, or (iii) $Pr(D_{j\ell}(z)-D_{j\ell}(z') = \mbox{sgn}(P(z)-P(z'))|Y_j(\ell)-Y_j(0)=Y_i(\ell)-Y_i(0)) \geq
Pr(D_{j\ell}(z)-D_{j\ell}(z') = -\mbox{sgn}(P(z)-P(z'))|Y_j(\ell)-Y_j(0)=Y_i(\ell)-Y_i(0))$ for all $\ell$.
\end{condition}
% \begin{condition}[Net Monotonicity]\label{net_monotonicity}
% For all $z,z'\in \mathcal{Z}$, either (i) $D_{i\ell}(z)-D_{i\ell}(z') = \mbox{sgn}(P(z)-P(z'))$, (ii) $D_{i\ell}(z)-D_{i\ell}(z') = 0$, or (iii) there exists a set $\mathcal{I}_{i\ell} \subseteq \mathcal{I}$ such that all $j \in \mathcal{I}_{i\ell}$ have $Y_j(\ell)-Y_j(0)=Y_i(\ell)-Y_i(0)$ and $Pr(D_{j\ell}(z)-D_{j\ell}(z') = \mbox{sgn}(P(z)-P(z'))|j \in \mathcal{I}_{i\ell}) \geq Pr(D_{i\ell}(z)-D_{i\ell}(z') = \mbox{sgn}(P(z)-P(z')))$     P_\ell(z') and a $z'' \in \mathcal{Z}$ such that $D_{j m}(z)-D_{j m}(z'')=\mbox{sgn}(P(z)-P(z'))$ and for some $m$ in $1,2,...,L$, for all $i$. 
% \end{condition}
% \begin{condition}[Net Monotonicity]\label{net_monotonicity}
% For all $z,z'\in \mathcal{Z}$, either (i) $D_{i\ell}(z)-D_{i\ell}(z') = \mbox{sgn}(P(z)-P(z'))$, (ii) $D_{i\ell}(z)-D_{i\ell}(z') = 0$, or (iii) there exists a $j$ and a $z'' \in \mathcal{Z}$ such that $D_{j m}(z)-D_{j m}(z'')=\mbox{sgn}(P(z)-P(z'))$ and $Y_j(m)-Y_j(0)=Y_i(\ell)-Y_i(0)$ for some $m$ in $1,2,...,L$, for all $i$. 
% \end{condition}
% \begin{condition}[Treatment Response Homogeneity]\label{net_monotonicity}
% For all $z,z'\in \mathcal{Z}$, either \\ $\mathbb{E}[D_{i\ell}(z)]\geq \mathbb{E}[D_{i\ell}(z')]$ for all $\ell$, or $\mathbb{E}[D_{i\ell}(z)]\leq \mathbb{E}[D_{i\ell}(z')]$ for all $\ell$.
% \end{condition}
Cases (i) and (ii) correspond to the monotonicity condition described by \cite{imbens1994identification}, extended to the current setting with multiple unobserved treatments. \cite{kline2016evaluating} describe a similar condition that restricts changes in the treatment decision to a single observed component treatment in the presence of multiple observed component treatments, while \cite{hull2018isolateing} describes a similar condition that restricts changes in treatment decision from one of multiple observed untreated states to a single observed component treatment. The relevant distinction in this paper is that even when (i) and (ii) hold for all individuals, my Condition \ref{net_monotonicity} still permits multiple unobserved types of treatment, wherein identified treatment effects are not only weighted averages of treatment effects for particular groups of individuals, but also for particular component treatments.

To better discuss case (iii), I adapt the language of \cite{angrist1996identification} to describe groups of individuals with respect to their component treatment statuses for different instrument comparisons. A component $\ell$ always-taker chooses component treatment $\ell$ regardless of their value for $Z_i$. A component $\ell$ never-taker never chooses component treatment $\ell$ regardless of their value for $Z_i$. Always takers for any component $\ell$ are necessarily never-takers for all other component treatments, as well as the untreated state. Component $\ell$ compliers at instrument comparison $z,z'$ have $D_{i\ell}(z)-D_{i\ell}(z') = \mbox{sgn}(P(z)-P(z'))$. Finally, component $\ell$ defiers at instrument comparison $z,z'$ have $D_{i\ell}(z)-D_{i\ell}(z') = -\mbox{sgn}(P(z)-P(z'))$.

Case (iii) of Condition \ref{net_monotonicity} essentially allows for defiers for any component as long as there are compliers for that component to cancel them out. When a subset of compliers cancel out defiers, the local treatment effect estimated at the instrument comparison will be driven by the residual subset of compliers that do not cancel out defiers. 
% A graphical illustration of the residual compliers is provided in Figure \ref{fig:residual_compliers} (placeholder for a link to a figure that shows Panel A, a frequency distribution over treatment effects, where the complier frequency is higher at all values of the support, and Panel B, the frequency distribution of compliers minus defiers at each point in the support).

To define this set of residual compliers more formally, I define the set of defiers for component treatment $\ell$ at $z,z'$ as $\mathcal{I}_{\ell}^{D;z,z'}$ and the set of compliers for component $\ell$  as $\mathcal{I}^{C;z,z'}_{\ell}$. I then partition the data such that $i=1,\dots,N_{D1} \in \mathcal{I}^{D;z,z'}_{1}, i=N_{D1}+1,\dots,N_{D1}+N_{C1} \in \mathcal{I}^{C;z,z'}_{1}, \dots , i=\sum_{\ell=1}^{L-1}N_{D\ell}+N_{C\ell}+1,\dots,\sum_{\ell=1}^{L-1}N_{D\ell}+N_{C\ell}+N_{DL} \in \mathcal{I}^{D;z,z'}_{L}$,
$i=\sum_{\ell=1}^{L-1}N_{D\ell}+N_{C\ell}+1,\dots,\sum_{\ell=1}^{L}N_{D\ell}+N_{C\ell} \in \mathcal{I}^{C;z,z'}_{L}$, where $N_{D\ell}$ is the number of defiers for component treatment $\ell$ and $N_{C\ell}$ is the number of compliers for component treatment $\ell$. In words, I order individuals such that defiers for component treatment 1 are first, followed by compliers for component treatment 1, then defiers for component 2, and so on (with always-takers and never-takers for all component treatments coming last). Within the set $\mathcal{I}^{D;z,z'}_{\ell}$ for each $\ell$, I order individuals such that $Y_{i}(\ell)-Y_{i}(0) \leq Y_{i+1}(\ell)-Y_{i+1}(0)$ for all $i \in \mathcal{I}^{D;z,z'}_{\ell}$. Within the set $\mathcal{I}^{C;z,z'}_{\ell}$, I order individuals such that $\sum_{i=N_{-\ell}+N_{D\ell}+1}^{N_{-\ell}+2N_{D\ell}}|(Y_{i}(\ell)-Y_{i}(0)) - (Y_{i-N_{D\ell}}(\ell)-Y_{i-N_{D\ell}}(0))|$ is minimized, where I define $N_{-\ell} = \sum_{m=1}^{\ell-1}N_{Dm}+N_{Cm}$. I define a residual complier for component treatment $\ell$ as an $i \in \mathcal{I}_{\ell}^{RC}$ for whom $i > N_{-\ell}+2N_{D\ell}$. In words, this ordering pairs each defier for component treatment $\ell$ with a complier for component treatment $\ell$ at the same position within the order of compliers, such that compliers that are not paired with a defier have relatively high values of the index $i$. Condition \ref{net_monotonicity} ensures that the minimum of $\sum_{i=N_{-\ell}+N_{D\ell}+1}^{N_{-\ell}+2N_{D\ell}}|(Y_{i}(\ell)-Y_{i}(0)) - (Y_{i-N_{D\ell}}(\ell)-Y_{i-N_{D\ell}}(0))|=0$ such that each defier-complier pair have equal treatment effects.

Other similar sufficient conditions exist for identification of positively-weighted local average component treatment effects. One is the existence of a value of the instrument $z$ such that $P(z)=0$ or $P(z)=1$, such that all comparisons of $z,z'\in \mathcal{Z}$ only include compliers for all component treatments, as discussed in the homogeneous treatment setting by \cite{heckman1990varieties} and \cite{angrist1991sources}.\footnote{The particular value of restricting individuals to these two cases is one advantage of randomized controlled trials.} An intuitively similar condition allows for defiers at some instrument comparisons as long as a sufficient mass of individuals with the same treatment effect are compliers at other instrument comparisons, as described in \cite{mogstad2021identification}.\footnote{The tests described in \cite{mogstad2021identification} to determine whether there are sufficient compliers at well-behaved instrument comparisons to cancel out noncompliers at poorly-behaved instrument comparisons are not immediately applicable to settings with unobserved treatment heterogeneity.} I concentrate on my Condition \ref{net_monotonicity} because cases (i) and (ii) are analogous to the commonly-invoked \cite{imbens1994identification} monotonicity condition, while case (iii) simplifies to the following under component treatment effect homogeneity:
\begin{condition}[Homogeneous Treatment Effects Net Monotonicity]\label{homogeneous_effects_net_monotonicity}
    (i) $Y_i(\ell)-Y_i(0) = \lambda_\ell$ for all  $i$ and (ii) for all $z,z'\in \mathcal{Z}$,  either
    $P_{\ell}(z)\geq P_{\ell}(z') $
    for all $\ell$,
    or $P_{\ell}(z)\leq P_{\ell}(z')$  for all  $\ell$.
\end{condition}
\noindent This condition preserves the logic of the IA monotonicity condition with the modification that the relevant compliers for instrument comparisons are component treatments rather than individuals.



We  can identify an average treatment effect of the composite treatment using instrumental variables by dividing the difference in outcomes at different values of instruments expressed in (\ref{Nonparametic_Reduced_Form_Decomposition}) by the net difference in the share of the population that chooses the composite treatment. Condition 2 ensures that this average treatment effect is a positively weighted average of underlying component treatment effects for a subset of the population of interest. Formally, I provide the following result:
\begin{thm}
    If Conditions \textnormal{\ref{existence_of_instruments}} and \textnormal{\ref{net_monotonicity}} hold, the average treatment effect defined by 
    \begin{equation*}
    \pi_{z,z'} = 
    \sum_{\ell=1}^L
    \theta_\ell
    \mathbb{E}
    \Big[
    Y_i(\ell)-Y_i(0)
    \Big|
    % D_{i\ell}(z) - D_{i\ell}(z') = sgn(P(z)-P(z')),
    i \in \mathcal{I}_\ell^{RC;z,z'}
    \Big]
    \end{equation*}
    % \begin{equation*}
    % \begin{split}
    % \frac{\mathbb{E}[Y_i|Z_i=z] - \mathbb{E}[Y_i|Z_i=z']}
    % {P(z)-P(z')}\\
    % &= 
    % \sum_{\ell=1}^L
    % \frac{
    % P_\ell(z)-P_\ell(z')
    % \lambda_\ell
    % }
    % {P(z)-P(z')
    % }
    % .
    % \end{split}
    % \end{equation*}
    % \begin{equation*}
    % \begin{split}
    % \pi_{z,z'} &= 
    % \frac{\mathbb{E}[Y_i|Z_i=z] - \mathbb{E}[Y_i|Z_i=z']}
    % {P(z)-P(z')}\\
    % &= 
    % \sum_{\ell=1}^L
    % \frac{
    % P_\ell(z)-P_\ell(z')
    % \lambda_\ell
    % }
    % {P(z)-P(z')}
    % .
    % \end{split}
    % \end{equation*}
    is identified from the joint distribution of $(Y,D,Z)$ and $\theta_\ell \in [0,1]$ for all $\ell=1,2,...,L$ for all $z,z'\in\mathcal{Z}$ such that $\mathbb{E}[Y_i|Z_i=z]$ and $\mathbb{E}[Y_i|Z_i=z']$ are finite and $P(z)\neq P(z')$, with  $\theta_\ell$ given by
    \begin{equation*}
        \theta_\ell = 
        \frac{
    P_\ell(z)-P_\ell(z')
    }
    {P(z)-P(z')
    }.
    \end{equation*}
\end{thm}

\begin{proof}
Let Condition \ref{existence_of_instruments} be satisfied. It follows that equation (\ref{Nonparametic_Reduced_Form_Decomposition}) holds. Using the sets defined above, this expression is equivalent to
\begin{equation*}
\begin{split}
    \mathbb{E}[Y_i&|Z_i=z] - \mathbb{E}[Y_i|Z_i=z'] \\
    = 
    % &
    &\sum_{\ell=1}^L 
    \Pr(i\in \mathcal{I}_\ell^{RC;z,z'})\mathbb{E}[Y_i(\ell)-Y_i(0)|i\in \mathcal{I}_\ell^{RC;z,z'}] \\
    +
    &\sum_{\ell=1}^L \Pr(i\in \mathcal{I}_\ell^C,i\not\in \mathcal{I}_\ell^{RC;z,z'})\mathbb{E}[Y_i(\ell)-Y_i(0)|i\in \mathcal{I}_\ell^C,i\not\in \mathcal{I}_\ell^{RC;z,z'}] \\
    - 
    &\sum_{\ell=1}^L \Pr(i\in \mathcal{I}_\ell^{D;z,z'})\mathbb{E}[Y_i(\ell)-Y_i(0)|i\in \mathcal{I}_\ell^{D;z,z'}].
    %
    % \mathbb{E}\Big[(D_{i\ell}(z)-D_{i\ell}(z'))(Y_i(\ell)-Y_i(0)) \Big],
    \end{split}
\end{equation*}
Let Condition \ref{net_monotonicity} be satisfied as well. It follows from the definitions of the sets $\mathcal{I}_\ell^{D;z,z'}$, $\mathcal{I}_\ell^{C;z,z'}$, and $\mathcal{I}_\ell^{RC;z,z'}$  that the last two lines of the above expression cancel out, yielding
\begin{equation*}
\begin{split}
    \mathbb{E}[Y_i&|Z_i=z] - \mathbb{E}[Y_i|Z_i=z'] \\
    = 
    % &
    &\sum_{\ell=1}^L 
    \Pr(i\in \mathcal{I}_\ell^{RC;z,z'})\mathbb{E}[Y_i(\ell)-Y_i(0)|i\in \mathcal{I}_\ell^{RC;z,z'}].
    \end{split}
\end{equation*}
Given that $D_{i\ell}(z)-D_{i\ell}(z') \neq 0$ iff $i\in \mathcal{I}_\ell^{C;z,z'}$ or $i\in \mathcal{I}_\ell^{D;z,z'}$, it follows that $\Pr(i\in \mathcal{I}_\ell^{RC;z,z'}) = P_\ell(z)-P_\ell(z')$. Making this substitution and multiplying the right-hand side of the equation by $(P(z)-P(z'))/(P(z)-P(z'))$ gives
\begin{equation*}
\begin{split}
    \mathbb{E}[Y_i&|Z_i=z] - \mathbb{E}[Y_i|Z_i=z'] \\
    = 
    % &
    &
    (P(z)-P(z'))\sum_{\ell=1}^L 
    \frac{
    P_\ell(z)-P_\ell(z')
    }
    {
    P(z)-P(z')
    }
    \mathbb{E}[Y_i(\ell)-Y_i(0)|i\in \mathcal{I}_\ell^{RC;z,z'}].
    \end{split}
\end{equation*}
Dividing each side of the equation by $(P(z)-P(z'))$ shows that the local component average treatment effect $\pi_{z,z'}$ is identified in terms of moments of the distribution of $(Y,D,Z)$.
\end{proof}





% Case (iii) allows for component treatment defiers so long as they are cancelled out by compliers who share their treatment effects. The case in which defiers at some instrument comparisons are compliers at other instrument comparisons is a multi-treatment extension of the partial monotonicity assumption described by \cite{mogstad2021identification}. I also allow for the case in which different groups of individuals at the same (or different) instrument comparisons happen to have the same treatment effects as the defiers for the component treatment they move out of. This can occur in three main ways, two of which are relatively straightforward. The first is the case in which an individual switches between component treatments that share the same idiosyncatic effect for them, in which case they are a complier for one component treatment that cancels out a defier for another (themselves). The second is the case of homogeneous component treatment effects, in which all that is necessary is that all aggregate changes in component treatment shares match the sign of the change in composite treatment.\footnote{The homogeneous component treatment effect version of Condition 2 can be constructed by removing (iii) and substituting $P$ in for $D_i$ throughout the statement of the condition.} Finally, it is possible that complier individuals at the same or different instrument value comparisons happen to have the same treatment effects at their chosen component treatments as the defiers had at the component treatments for which they are defiers.

Figure \ref{fig:Net_monotonicity_illustration} shows a graphical illustration of the decision setting. The horizontal axes give a latent utility index for the composite treatment, such that the composite treatment is chosen if $V_i\geq0$. The vertical axes give a relative preference for two component treatments, such that treatment 1 is chosen if $V_{1i} \geq 0$ and $V_i\geq0$, and treatment 2 is chosen if $V_{11} < 0$ and $V_i\geq0$. The ovals drawn in each figure contain uniform joint distributions of individuals' preferences for treatments. Each panel shows a different instrument comparison assumed to satisfy Condition \ref{existence_of_instruments}. The instrument shift in panel A satisfies Condition \ref{net_monotonicity} without any individual defiers for any component treatment. The shift in panel B satisfies Condition \ref{net_monotonicity} under a homogeneous component treatment effects assumption, while the shift in panel C does not. 
% In each case, Condition \ref{net_monotonicity} may be satisfied if the treatment effects of compliers happen to match those of defiers for the component treatment for which they are a defier.%
%\footnote{Note that if the two component treatments have the same effects for each individual, Condition \ref{net_monotonicity} will be trivially satisfied for each instrument shown.}




%\newgeometry{margin=1cm} % modify this if you need even more space
%\begin{landscape}
\begin{SidewaysFigure}

    \centering
    \begin{subfigure}[t]{0.4\textwidth}
    \raggedright
        Panel A
        \begin{center}
        \resizebox{\textwidth}{!}{
\begin{tikzpicture}
\node[label=below:{$D=0$} ]   () at (-3.0, -2) {};
\node[label=above:{$D=0$} ]   () at (-3.0, 2) {};
\node[label=below:{$D_{2}=1$} ]   () at (3.0, -2) {};
\node[label=above:{$D_{1}=1$} ]   () at (3.0, 2) {};
\node[label=below:{$V$} ]   () at (3.5, 0) {};
\node[label=right:{$V_1$} ]   () at (0, 2.5) {};
\node[label=above:z']   () at (.6, -.7) {};
\node[label=above:z]   () at (1.3, -.7) {};

\draw [-{Latex[round]}] (0,0) -- (0,3);
\draw [-{Latex[round]}] (0,0) -- (0,-3);
\draw[white, thick] (-4,0) -- (0,0); %To center
\draw [-{Latex[round]}] (0,0) -- (4,0);
\draw [-{Latex[round]}] (0,0) -- (-4,0);
\draw[rotate=45][gray, dashed] (-1,0) ellipse (60pt and 30pt);
\draw [-{Latex[round]}] (0,0) -- (0,-3);
\draw[rotate=45] (-.5,-.5) ellipse (60pt and 30pt);
\draw [-{Latex[round]}] (.7,-.6) -- (1.4,-.6);
\end{tikzpicture}
}
\end{center}
\end{subfigure}
\hspace{0.05\textwidth}%
%
%
%
%
    \begin{subfigure}[t]{0.4\textwidth}
    \raggedright
        Panel B
        \begin{center}
        \resizebox{\textwidth}{!}{
\begin{tikzpicture}
\node[label=below:{$D=0$} ]   () at (-3.0, -2) {};
\node[label=above:{$D=0$} ]   () at (-3.0, 2) {};
\node[label=below:{$D_{2}=1$} ]   () at (3.0, -2) {};
\node[label=above:{$D_{1}=1$} ]   () at (3.0, 2) {};
\node[label=below:{$V$} ]   () at (3.5, 0) {};
\node[label=right:{$V_1$} ]   () at (0, 2.5) {};
\node[label=below:z']   () at (.8, .8) {};
\node[label=below:z]   () at (1.5, 1.5) {};

\draw [-{Latex[round]}] (0,0) -- (0,3);
\draw [-{Latex[round]}] (0,0) -- (0,-3);
\draw[white, thick] (-4,0) -- (0,0); %To center
\draw [-{Latex[round]}] (0,0) -- (4,0);
\draw [-{Latex[round]}] (0,0) -- (-4,0);
\draw[rotate=45][gray, dashed] (-1,0) ellipse (60pt and 30pt);
\draw [-{Latex[round]}] (0,0) -- (0,-3);
\draw[rotate=45] (0,0) ellipse (60pt and 30pt);
\draw [-{Latex[round]}] (.8,.8) -- (1.5,1.5);
\end{tikzpicture}
}
\end{center}
\end{subfigure}
\hspace{0.05\textwidth}%
%
%
%
    \begin{subfigure}[t]{0.4\textwidth}
    \raggedright
        Panel C
        \begin{center}
        \resizebox{\textwidth}{!}{
\begin{tikzpicture}
\node[label=below:{$D=0$} ]   () at (-3.0, -2) {};
\node[label=above:{$D=0$} ]   () at (-3.0, 2) {};
\node[label=below:{$D_{2}=1$} ]   () at (3.0, -2) {};
\node[label=above:{$D_{1}=1$} ]   () at (3.0, 2) {};
\node[label=below:{$V$} ]   () at (3.5, 0) {};
\node[label=right:{$V_1$} ]   () at (0, 2.5) {};
\node[label=below:z']   () at (0.2,-1.4) {};
\node[label=below:z]   () at (.8,-2.1) {};

\draw [-{Latex[round]}] (0,0) -- (0,3);
\draw [-{Latex[round]}] (0,0) -- (0,-3);
\draw[white, thick] (-4,0) -- (0,0); %To center
\draw [-{Latex[round]}] (0,0) -- (4,0);
\draw [-{Latex[round]}] (0,0) -- (-4,0);
\draw[rotate=45][gray, dashed] (-1,0) ellipse (60pt and 30pt);
\draw [-{Latex[round]}] (0,0) -- (0,-3);
\draw[rotate=45] (-1,-1) ellipse (60pt and 30pt);
\draw [-{Latex[round]}] (0.1,-1.4) -- (.8,-2.1);
\end{tikzpicture}
}
\end{center}
\end{subfigure}
\caption{Instrument Comparisons with Two Unobserved Component Treatments}
\label{fig:Net_monotonicity_illustration}
   \begin{minipage}{1\linewidth}
\smallskip
\footnotesize
\emph{Notes:} For composite treatment preference $V$ and relative preference for component treatment 1 $V_1$, each panel shows a different instrument comparison. Panel A depicts an instrument comparison where individuals' preference for treatment increases, but there is no effect on the composition of treatment (no defiers). Panel B shows a comparison where more individuals choose each type of treatment at $z$ than at $z'$, but there are compositional changes in the individuals who choose each component treatment. If component treatment effects are homogeneous, the situation in Panel B will satisfy my Net Monotonicity condition. Panel C depicts an instrument comparison where the aggregate composition of treatment shifts in response to the treatment. Net monotonicity will only hold in this setting if the idiosyncratic treatment effects of compliers cancel out the treatment effects for the group of people who shift from component treatment 1 to component treatment 2, for instance if component 1 and component 2 have identical treatment effects for defiers.
\end{minipage}
\end{SidewaysFigure}

%\end{landscape}
%\restoregeometry

The assumption that no individuals switch their preferred version of treatment in response to instruments may be strong in many settings, even those in which Imbens and Angrists' monotonicity assumption is uncontroversial. For instance, an instrument that reduces costs for college may produce income effects, which may cause some students to obtain leisure by choosing lower-earnings majors%
%\citep{leslie turner}
. It may seem similarly strong to assume that there happen to be compliers that exactly cancel out defiers as I describe in case (iii) of Condition \ref{net_monotonicity}. However, if treatment composition shifts are small relative to net shifts in treatment, the number of compliers who are available to cancel out defiers will be relatively large. If the defier treatment effect distribution is encompassed by the support of the complier treatment effect distribution, Condition \ref{net_monotonicity} will be satisfied if compliers sufficiently outnumber defiers. The economic content of such an assumption is that instrumental variables cause shifts in observed composite treatments that are large relative to unobserved component treatment shifts, which seems likely to be satisfied in many settings where a strict person-specific component treatment monotonicity condition would be violated.




% To fix ideas, I take the opportunity to describe a policy-relevant example of an instrument that. Consider a policy that gives students a large college scholarship that is contingent on the student pursing humanities coursework. Suppose further that the wage return to the humanities type of college education is half that of the wage return to non-humanities college (saying nothing about non-wage returns). It is very likely that such a policy, if well-publicized, would have a strong first stage, reflecting its effect on shifting individuals into college. Furthermore, it is likely that such a policy would also induce some students who planned on pursuing non-humanities coursework to instead pursue humanities course work. Using the implementation of this policy as an instrumental variable for the return to college, therefore, would then result in estimates of the return to college that would be below those for both humanities college education and non-humanities college education.
